Byzantine Fault-Tolerant Distributed Machine Learning Using Stochastic Gradient Descent (SGD) and Norm-Based Comparative Gradient Elimination (CGE)

This paper considers the Byzantine fault-tolerance problem in distributed stochastic gradient descent (D-SGD) method - a popular algorithm for distributed multi-agent machine learning. In this problem, each agent samples data points independently from a certain data-generating distribution. In the fault-free case, the D-SGD method allows all the agents to learn a mathematical model best fitting the data collectively sampled by all agents. We consider the case when a fraction of agents may be Byzantine faulty. Such faulty agents may not follow a prescribed algorithm correctly, and may render traditional D-SGD method ineffective by sharing arbitrary incorrect stochastic gradients. We propose a norm-based gradient-filter, named comparative gradient elimination (CGE), that robustifies the D-SGD method against Byzantine agents. We show that the CGE gradient-filter guarantees fault-tolerance against a bounded fraction of Byzantine agents under standard stochastic assumptions, and is computationally simpler compared to many existing gradient-filters such as multi-KRUM, geometric median-of-means, and the spectral filters. We empirically show, by simulating distributed learning on neural networks, that the fault-tolerance of CGE is comparable to that of existing gradient-filters. We also empirically show that exponential averaging of stochastic gradients improves the fault-tolerance of a generic gradient-filter.

==> correctness-dsn-dsml.tex <==
\subsection{Fault-Tolerance Property}
\label{sec:ft}
In this section, we present a formal convergence result for our algorithm under assumptions, stated below, that hold true in most learning problems~\cite{bottou2018optimization}. \\

For each non-faulty agent $i$, let 
    \( \z^t_i = \{z^t_{i_1}, \ldots, \, z^t_{i_k}\}\), 
    denote the collection of $k$ i.i.d.~data points sampled by the agent $i$ in iteration $t$. Now, for each agent $i$ and iteration $t$ we define a random variable 
    \begin{align}
        \zeta^t_i = \left\{ \begin{array}{ccc} \z^t_i & , & \text{agent $i$ is non-faulty} \\ g^t_i & , & \text{agent $i$ is faulty}\end{array}\right. \label{eqn:def_zeta_i}
    \end{align}
    Recall that~$g^t_i$ may be an arbitrary $d$-dimensional random variable for each Byzantine faulty agent $i$. For each iteration $t$, let
        \( \zeta^t = \{\zeta^t_i, ~ i = 1, \ldots, \, n\} \), 
    and let $\E_t$ denote the expectation with respect to the collective random variables $\zeta^0, \ldots, \, \zeta^t$, given the initial estimate $w^0$. Specifically, 
    %\begin{align}
      \(  \E_t(\cdot) = \E_{\zeta^0, \ldots, \, \zeta^{t}} (\cdot),\,\forall t \geq 0 \).

\begin{assumption}[Bounded variance]
\label{asp:bnd_var}
% For each non-faulty agent $i$, assume that the variance of $g^t_i$ is bounded. Specifically, 
Assume that there exists a finite real value $\sigma$ such that for all non-faulty agent $i$,
\[\E_{\zeta^t_i} \norm{ g^t_i - \E_{\zeta^t_i} \left(g^t_i\right)}^2 \leq \sigma^2, \quad \forall t.\]
\end{assumption}

\begin{assumption}[Lipschitz smoothness]
\label{asp:lip}
Assume that there exists a finite positive real value $\mu$ such that
\begin{align*}
    \norm{\nabla Q(w) - \nabla Q(w')} \leq \mu \norm{w - w'}, \quad \forall w, \, w' \in \R^d.
\end{align*}
\end{assumption}

\begin{assumption}[Strong convexity]
\label{asp:str_cvx}
Assume that there exists a finite positive real value $\lambda$ such that for all $w, \, w' \in \R^d$,
\begin{align*}
    \iprod{w - w'}{\nabla Q(w) - \nabla Q(w')} \geq \lambda \norm{w - w'}^2.
\end{align*}
\end{assumption}

% First, we introduce some notation.
% In particular, we assume that the stochastic gradients have bounded variance, the gradient function $\nabla Q(w)$ is Lipschitz continuous, and that the expected loss function $Q(w)$ is strongly convex. Our assumptions are formally listed below.\\
We define a {\em fault-tolerance margin}  
    \begin{align}
        \alpha = \frac{\lambda}{2\lambda + \mu} - \frac{f}{n} \label{eqn:alpha_learn}
    \end{align}
    that determines the maximum fraction of faulty agents $f/n$ tolerable by our algorithm. Lastly, we define an upper bound for the step-size $\eta_t$ in~\eqref{eqn:algo_1},
    \begin{align}
        \overline{\eta} = \left(\frac{2(2 \lambda + \mu)n}{n^2 + (n-f)^2 \mu^2 } \right) \, \alpha. \label{eqn:step_learn}
    \end{align}
    % The meaning of $\mu$ and $\lambda$ are introduced later.
    
% \begin{itemize}
%     \item  %\label{eqn:notation_exp}
%     %\end{align}
%     \item 
%     % \item Let
%     % \begin{align}
%     %     \M^2 = \left(\frac{f^2 \left( 1 + \sqrt{n-f-1}\right)^2}{n^2} + \eta^2 (n-f)^2 \right) \sigma^2. \label{eqn:ss_error}
%     % \end{align}
% \end{itemize}

% We make the following assumptions that are satisfied in many machine learning problems~\cite{bottou2018optimization, yin2018byzantine}.
% Our convergence result relies on 
% Our assumptions are formally listed below. In Theorem~\ref{thm:conv}, following the assumptions, we present our key result on the convergence of our algorithm, i.e., Algorithm~\ref{alg:cge}.\\




% As noted by~\cite{bottou2018optimization}, the assumption on strong convexity of $Q(w)$ is not very restrictive in the practical scenarios of machine learning. For instance, in many situations when a convex learning model is used -- such as logistic regression or support vector machine -- it is often regularized by a strongly
% convex function. Moreover, even if the global cost $Q(w)$ is not strongly convex over the entire search space $\R^d$, it is so in the neighborhood of local minimizers. This means that our algorithm can guarantee fault-tolerance in small regions of the learning parameter search space.\\

Theorem~\ref{thm:conv} below presents a key fault-tolerance property of our Algorithm~\ref{alg:cge}. Recall that 
% $w^*$ denotes a minimum of the global expected loss function $Q(w)$
% , i.e.,
\(w^* \in \arg \min_{w \in \R^d} Q(w).\)

\begin{theorem} 
\label{thm:conv}
Consider Algorithm~\ref{alg:cge}. Suppose that the Assumptions~\ref{asp:bnd_var},~\ref{asp:lip}, and~\ref{asp:str_cvx} hold true. If the fault-tolerance margin $\alpha$ is positive, and in the update law~\eqref{eqn:algo_1} the step-size $\eta_t = \eta \in \left(0, ~ \overline{\eta} \right)$ for all $t$ then 
\begin{align}
    \rho  = 1 - \left(n^2 + (n-f)^2 \mu^2 \right) \, \eta \left( \overline{\eta} - \eta \right) \in (0, ~ 1), \label{eqn:rho}
\end{align}
and, for all $t \geq 1$, 
\begin{align}
    \E_{t-1} \norm{w^{t} - w^*}^2 \leq \rho^{t} \norm{w^{0} - w^*}^2 + \left(\frac{1 - \rho^{t}}{ 1- \rho}\right) \M^2 \label{eqn:rate}
\end{align}
where
%\begin{align}
  \(  \M^2 = \left(\dfrac{f^2 \left( 1 + \sqrt{n-f-1}\right)^2}{n^2} + \eta^2 (n-f)^2 \right) \sigma^2 \). %\label{eqn:ss_error}
%\end{align}
\end{theorem}
% The proof of Theorem~\ref{thm:conv} can be found in the  deferred to Appendix~\ref{app:pf_thm}.\\
The proof is omitted due to the space constraint, and can be found in the full version on arXiv \cite{gupta2020byzantine}.

According to Theorem~\ref{thm:conv}, if $\alpha > 0$, i.e., 
\(    \dfrac{f}{n} < \cfrac{\lambda}{2\lambda + \mu}\), % \label{eqn:bnd_fn}
then for small enough step-size, in~\eqref{eqn:algo_1}, our algorithm converges {\em linearly} to a neighborhood of a minimum of the global expected loss function~\eqref{eqn:exp_loss}. As $\rho < 1$,~\eqref{eqn:rate} implies that
\[\lim_{t \to \infty} \E_{t-1} \norm{w^{t} - w^*}^2 \leq \frac{\M^2}{ 1- \rho}. \]
Upon using the Markov's inequality, we obtain the probabilistic guarantee on training accuracy stated in Section~\ref{sub:contri}.
% statement corollary of Theorem~\ref{thm:conv}. Notation $Pr$ stands for probability. 

% \begin{corollary}
% \label{cor:learn}
% Consider Algorithm~\ref{alg:cge}. If the conditions stated in Theorem~\ref{thm:conv} hold true then
% for all $\epsilon > 0$,
% \[\lim_{t \to \infty} Pr \left( \norm{w^t - w^*}^2 \leq \epsilon \right) \geq 1 - \frac{1}{\epsilon} ~ \left( \frac{\M^2}{1 - \rho}\right). \]
% \end{corollary}

% % The proof for Corollary~\ref{cor:learn}, presented in Appendix~\ref{app:cor_learn}, relies on Markov's inequality. In the subsequent section, we present the formal proof for Theorem~\ref{thm:conv}.\\

% According to Corollary~\ref{cor:learn}, the D-SGD method in conjunction with our CGE gradient-filer converges within $\epsilon$ distance to an optimal learning parameter with probability at least 
% \[1 - \frac{1}{\epsilon} ~ \left( \frac{\M^2}{1 - \rho}\right),\]
% despite the presence of up to $f$ Byzantine faulty agents. \\

% We discuss below the trade-off between the DP of the gradients in each iteration and the asymptotic learning accuracy of our
% The value of $\M^2$, defined in~\eqref{eqn:ss_error}, is proportional to the variance $\sigma^2$ of the non-faulty stochastic gradients. Thus, we obtain improved fault-tolerance when the non-faulty stochastic gradients have smaller variances, or less noise.\\
% a higher probability of estimating an optimal learning parameter within $\epsilon$ error.\\
% Note that the stochastic gradients are unbiased estimators of the true gradient of the global expected loss function, as shown in Section~\ref{sub:s_grad}. Smaller is the variance $\sigma^2$, the more accurate are the stochastic gradients (see Assumption~\ref{asp:bnd_var}). Therefore, it is quite intuitive that fault-tolerance of the proposed algorithm should improve when the accuracy of the stochastic gradients computed by the non-faulty agents improves.\\

% Next, we present experimental results on the fault-tolerance of our algorithm when applied to distributed learning of artificial neural networks. 
% We compare the fault-tolerance achieved by our CGE gradient-filter with that of the other existing gradient-filters, namely multi-KRUM~\cite{blanchard2017machine}, geometric median of means~\cite{chen2017distributed}, and coordinate-wise trimmed mean~\cite{yin2018byzantine, su2018finite}. 



==> experiment_backup.tex <==
%====================
\iffalse
\subsubsection{Comparison among fraction of faulty agents}

It is also interesting to see how performance changes. Figure~\ref{fig:fraction-faults-1} shows the comparison using different filters under \textit{coordinate-wise} type of fault and batch size of 16.

\begin{figure}[t]
    \centering
    \subcaptionbox{Geometric median}{
    \includegraphics{Experiments/new/fault_fraction_comparison/loss-mnist-16-cwtm-geomedian-faults.pdf}
    \includegraphics{Experiments/new/fault_fraction_comparison/prec1-mnist-16-cwtm-geomedian-faults.pdf}
    \includegraphics{Experiments/new/fault_fraction_comparison/prec3-mnist-16-cwtm-geomedian-faults.pdf}\vspace{-8pt}
    }
    \subcaptionbox{Median of means}{
    \includegraphics{Experiments/new/fault_fraction_comparison/loss-mnist-16-cwtm-medofmeans-faults.pdf}
    \includegraphics{Experiments/new/fault_fraction_comparison/prec1-mnist-16-cwtm-medofmeans-faults.pdf}
    \includegraphics{Experiments/new/fault_fraction_comparison/prec3-mnist-16-cwtm-medofmeans-faults.pdf}\vspace{-8pt}
    }
    \subcaptionbox{Coordinate-wise trimmed mean}{
    \includegraphics{Experiments/new/fault_fraction_comparison/loss-mnist-16-cwtm-cwtm-faults.pdf}
    \includegraphics{Experiments/new/fault_fraction_comparison/prec1-mnist-16-cwtm-cwtm-faults.pdf}
    \includegraphics{Experiments/new/fault_fraction_comparison/prec3-mnist-16-cwtm-cwtm-faults.pdf}\vspace{-8pt}
    }
    \subcaptionbox{Multi-KRUM (m=2)}{
    \includegraphics{Experiments/new/fault_fraction_comparison/loss-mnist-16-cwtm-mkrum2-faults.pdf}
    \includegraphics{Experiments/new/fault_fraction_comparison/prec1-mnist-16-cwtm-mkrum2-faults.pdf}
    \includegraphics{Experiments/new/fault_fraction_comparison/prec3-mnist-16-cwtm-mkrum2-faults.pdf}\vspace{-8pt}
    }
    \subcaptionbox{CGE}{
    \includegraphics{Experiments/new/fault_fraction_comparison/loss-mnist-16-cwtm-normfilter-faults.pdf}
    \includegraphics{Experiments/new/fault_fraction_comparison/prec1-mnist-16-cwtm-normfilter-faults.pdf}
    \includegraphics{Experiments/new/fault_fraction_comparison/prec3-mnist-16-cwtm-normfilter-faults.pdf}\vspace{-8pt}
    }
    \caption{Comparison among different fraction of faulty agents.}
    \label{fig:fraction-faults-1}
\end{figure}
\fi

%\subsubsection{Accumulative approace for fault tolerance}

%Plan: adjust alpha

%\subsubsection{Different dataset}

%Plan: CIFAR-10

\iffalse
\begin{table}[t]
    \centering
    \tiny
    \begin{tabular}{|ccccccccc|}
        \hline
        \# agents & \# faulty & Dataset & Batch-size & Fault type & Methods & Network & Dataset & Comments \\
        \hline
        \hline
        40 & 10 & MNIST & 16 & All five & All five & LeNet & MNIST & \\
        40 & 5 & MNIST & 16 & All five & All five & LeNet & MNIST & \\
        \hline
        40 & 10 & MNIST & 16 & Krum/CGE & Concatenation & LeNet & MNIST & \\
        40 & 5 & MNIST & 16 & Krum/CGE & Concatenation & LeNet & MNIST & \\
        \hline
        40 & 0 & MNIST & 16 & N/A & Averaging & LeNet & MNIST & \\
        \hline
        \hline
        40 & 10 & MNIST & 64 & All five & All five & LeNet & MNIST & \\
        40 & 5 & MNIST & 64 & All five & All five & LeNet & MNIST & \\
        \hline
        40 & 10 & MNIST & 64 & Krum/CGE & Concatenation & LeNet & MNIST & \\
        40 & 5 & MNIST & 64 & Krum/CGE & Concatenation & LeNet & MNIST & \\
        \hline
        40 & 0 & MNIST & 64 & N/A & Averaging & LeNet & MNIST & \\
        \hline
    \end{tabular}
    \caption{List of experiment that we conduct.}
    \label{tab:experiment-plans}
\end{table}
\fi

\iffalse
\subsection{Results and analysis}

\subsubsection{Comparison between the five filters}

We conducted our experiments in batch-sizes of 16 and 64, and with number of faulty agents 5 and 10. Given the fact that there are 10 classes, it is expected that the smaller the batch-size, the more likely that samples drawn by different agents are from different classes, and therefore the gradients from different agents have higher variance. This might lead to different performance for some of the filters. As for the number of faults, we run experiments that make the server tolerate exactly the actual number of faults. It is expected that generally, the more the number of faulty agents, the worse the filters would perform.

\begin{figure}[t]
    \centering
    \subcaptionbox{Loss}{
        \begin{minipage}{0.31\linewidth}
        \includegraphics[width=\linewidth]{Experiments/mnist-16-5/loss-mnist-16-5-geomedian.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-16-5/loss-mnist-16-5-medofmeans.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-16-5/loss-mnist-16-5-cwtm.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-16-5/loss-mnist-16-5-krum2.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-16-5/loss-mnist-16-5-normfilter.pdf}
        \end{minipage}
    }
    \subcaptionbox{Prec@1}{
        \begin{minipage}{0.31\linewidth}
        \includegraphics[width=\linewidth]{Experiments/mnist-16-5/prec1-mnist-16-5-geomedian.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-16-5/prec1-mnist-16-5-medofmeans.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-16-5/prec1-mnist-16-5-cwtm.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-16-5/prec1-mnist-16-5-krum2.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-16-5/prec1-mnist-16-5-normfilter.pdf}
        \end{minipage}
    }
    \subcaptionbox{Prec@3}{
        \begin{minipage}{0.31\linewidth}
        \includegraphics[width=\linewidth]{Experiments/mnist-16-5/prec3-mnist-16-5-geomedian.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-16-5/prec3-mnist-16-5-medofmeans.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-16-5/prec3-mnist-16-5-cwtm.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-16-5/prec3-mnist-16-5-krum2.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-16-5/prec3-mnist-16-5-normfilter.pdf}
        \end{minipage}
    }
    \caption{Comparison between five filters under five type of filters. Batch-size: 16; number of faults: 5. Each row from left to right are (a) Loss, (b) Precision at 1, and (c) Precision at 3 on testing dataset of MNIST. Type of faults from top to bottom: (1) Geometric median, (2) Median of means, (3) Coordinate-wise trimmed mean, (4) Multi-KRUM, and (5) CGE, as we discussed in Section \ref{sub:implementation-and-setup}.}
    \label{fig:experiment-results-1}
\end{figure}

Figure \ref{fig:experiment-results-1} shows the results of this comprehensive comparison with batch-size of 16 and 5 out of 40 faulty agents. As we can see, \emph{geomedian}, \emph{medofmeans}, and \emph{normfilter} are relatively ``easy'' types of faults for the filters, the fault-tolerant results are close to the fault-free case. \emph{Cwtm} and \emph{mkrum} are relatively ``difficult'', with many filters perform unstable. Over three types of faults, we observe that multi-KRUM converges slower than other type of filters, and CGE converges faster; for \emph{cwtm}, only median of means works stable; for \emph{mkrum}, multi-KRUM and CGE cannot converge. Figure \ref{fig:experiment-results-2} shows results with batch-size of 16 and 10 out of 40 faulty agents. With larger fraction of faulty agents, it is more difficult for all filters under all type of faults to tolerate. We can see that the optimization procedures converge slower comparing to less fault cases; while multi-KRUM and CGE losses become exponential much faster under \emph{mkrum} type of fault.

\begin{figure}[t]
    \centering
    \subcaptionbox{Loss}{
        \begin{minipage}{0.31\linewidth}
        \includegraphics[width=\linewidth]{Experiments/mnist-16-10/loss-mnist-16-10-geomedian.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-16-10/loss-mnist-16-10-medofmeans.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-16-10/loss-mnist-16-10-cwtm.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-16-10/loss-mnist-16-10-krum2.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-16-10/loss-mnist-16-10-normfilter.pdf}
        \end{minipage}
    }
    \subcaptionbox{Prec@1}{
        \begin{minipage}{0.31\linewidth}
        \includegraphics[width=\linewidth]{Experiments/mnist-16-10/prec1-mnist-16-10-geomedian.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-16-10/prec1-mnist-16-10-medofmeans.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-16-10/prec1-mnist-16-10-cwtm.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-16-10/prec1-mnist-16-10-krum2.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-16-10/prec1-mnist-16-10-normfilter.pdf}
        \end{minipage}
    }
    \subcaptionbox{Prec@3}{
        \begin{minipage}{0.31\linewidth}
        \includegraphics[width=\linewidth]{Experiments/mnist-16-10/prec3-mnist-16-10-geomedian.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-16-10/prec3-mnist-16-10-medofmeans.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-16-10/prec3-mnist-16-10-cwtm.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-16-10/prec3-mnist-16-10-krum2.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-16-10/prec3-mnist-16-10-normfilter.pdf}
        \end{minipage}
    }
    \caption{Comparison between five filters under five type of filters. Batch-size: 16; number of faults: 10. Each row from left to right are (a) Loss, (b) Precision at 1, and (c) Precision at 3 on testing dataset of MNIST. Type of faults from top to bottom: (1) Geometric median, (2) Median of means, (3) Coordinate-wise trimmed mean, (4) Multi-KRUM, and (5) CGE, as we discussed in Section \ref{sub:implementation-and-setup}.}
    \label{fig:experiment-results-2}
\end{figure}

\begin{figure}[t]
    \centering
    \subcaptionbox{Loss}{
        \begin{minipage}{0.31\linewidth}
        \includegraphics[width=\linewidth]{Experiments/mnist-64-5/loss-mnist-64-5-geomedian.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-64-5/loss-mnist-64-5-medofmeans.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-64-5/loss-mnist-64-5-cwtm.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-64-5/loss-mnist-64-5-krum2.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-64-5/loss-mnist-64-5-normfilter.pdf}
        \end{minipage}
    }
    \subcaptionbox{Prec@1}{
        \begin{minipage}{0.31\linewidth}
        \includegraphics[width=\linewidth]{Experiments/mnist-64-5/prec1-mnist-64-5-geomedian.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-64-5/prec1-mnist-64-5-medofmeans.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-64-5/prec1-mnist-64-5-cwtm.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-64-5/prec1-mnist-64-5-krum2.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-64-5/prec1-mnist-64-5-normfilter.pdf}
        \end{minipage}
    }
    \subcaptionbox{Prec@3}{
        \begin{minipage}{0.31\linewidth}
        \includegraphics[width=\linewidth]{Experiments/mnist-64-5/prec3-mnist-64-5-geomedian.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-64-5/prec3-mnist-64-5-medofmeans.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-64-5/prec3-mnist-64-5-cwtm.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-64-5/prec3-mnist-64-5-krum2.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/mnist-64-5/prec3-mnist-64-5-normfilter.pdf}
        \end{minipage}
    }
    \caption{Comparison between five filters under five type of filters. Batch-size: 64; number of faults: 5. Each row from left to right are (a) Loss, (b) Precision at 1, and (c) Precision at 3 on testing dataset of MNIST. Type of faults from top to bottom: (1) Geometric median, (2) Median of means, (3) Coordinate-wise trimmed mean, (4) Multi-KRUM, and (5) CGE, as we discussed in Section \ref{sub:implementation-and-setup}.}
    \label{fig:experiment-results-3}
\end{figure}

Figure \ref{fig:experiment-results-3} shows the experiments run with batch-size of 64 and number of faulty agent 5. Most behaviors of filters are similar comparing to batch-size of 16 version. It is expected, and as we can observe, that larger batch-size lead to faster convergence. One interesting observation other than this is multi-KRUM works better in the sense of convergence rate. The possible reason would be that the direction is less divergent with larger batch-size, which is helpful for multi-KRUM, a clustering-based filter, to tell which gradient is more likely to be faulty.


%%%%%%%%%%%%%%%%%%%%%%%% GRADIENT AVERAGING %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Gradient Averaging}
\label{sub:appendix_averaging}

We noticed that in previous experimental results, there are `unstable' behaviors shown in the plots, especially when under the fault type \textit{coordinate-wise}. We can see that in some cases, for example, $f=0$ or $1$ in Figure~\ref{fig:fault-fraction-1}(b), the minimums of loss during the training process can be very close to the corresponding fault-free loss at the same step, while there are pikes and turbulence once several steps. To address this problem, one possible way is to increase batch size. As is shown in Figure~\ref{fig:fault-fraction-3}(b), when batch size is increased from 16 to 64, although the pikes still exists, it become smaller and less frequent, thanks to the reduce of variance of the gradients.\\

Another way of address this problem might be using a gradient averaging scheme. By averaging previous steps gradients collected from each agent, it is expected to reduce variance among good agents, so that gradients from fault agents become more distinguishing to filters. Let $h^t_j$ denote the averaging history of gradients of agent $t$ at step $j$, $0\leq\alpha\leq1$,
$$h^t_j = \alpha\cdot h^{t-1}_j + (1-\alpha) g^t_j$$
Update parameters by the following scheme instead of:
$$w^t = w^{t-1} + \mu\cdot\mathrm{Filter}_j\{h^t_j\}$$
Note that under this definition, $\alpha=0$ indicates plain SGD with no averaging.\\

We conducted several experiments with the averaging scheme described above. Figure~\ref{fig:accumulation-1} and Figure~\ref{fig:accumulation-2} shows the results. The value of $\alpha$ varies between 0 and 0.60. Comparing plots in each figure, it is easy to find that with an increase of the value of $\alpha$, the pikes in loss (or dives in precision) become less significant and less frequent. Also, convergence speed does not change much with increasing of $\alpha$. In Figure~\ref{fig:accumulation-1}(b), we see that this averaging scheme can sometimes also helps SGD avoid a worse local minimum.\\

One thing worth noticing is that, the averaging scheme does not increase computation complexity by much.

\begin{figure}[p]
    \centering
    \includegraphics[width=\textwidth]{Experiments/new/accumulation_comparison/averaging-comparison-1.pdf}
    \caption{Comparison of different $\alpha$ values using averaging scheme, using filter multi-KRUM ($m=2$) with batch size 16, under fault type \textit{coordinate-wise}. Each row correspond to a different number of faults: (a) $f=1$, (b) $f=2$, (c) $f=3$, and (d) $f=4$.}
    \label{fig:accumulation-1}
\end{figure}
\begin{figure}[p]
    \centering
    \includegraphics[width=\textwidth]{Experiments/new/accumulation_comparison/averaging-comparison-2.pdf}
    \caption{Comparison of different $\alpha$ values using averaging scheme, using filter CGE with batch size 16, under fault type \textit{coordinate-wise}. Each row correspond to a different number of faults: (a) $f=1$, (b) $f=2$, (c) $f=3$, and (d) $f=4$.}
    \label{fig:accumulation-2}
\end{figure}
\begin{figure}[p]
    \centering
    \includegraphics[width=\textwidth]{Experiments/new/cifar_comparison/cifar-filter-comparison-1.pdf}
    \caption{Comparison of filters when training for CIFAR-10 dataset, using batch size 16, under fault type \textit{coordinate-wise}. Each row correspond to a different filter: (a) geometric median, (b) median of means, (c) coordinate-wise trimmed mean, (d) multi-KRUM ($m=2$), and (e) CGE.}
    \label{fig:cifar-1}
\end{figure}
\begin{figure}[p]
    \centering
    \includegraphics[width=\textwidth]{Experiments/new/cifar_comparison/cifar-averaging-comparison-1.pdf}
    \caption{Comparison of different $\alpha$ values using averaging scheme when training for CIFAR-10 dataset, using filter multi-KRUM ($m=2$) with batch size 16, under fault type \textit{coordinate-wise}. Each row correspond to a different number of faults: (a) $f=1$, (b) $f=2$, (c) $f=3$, and (d) $f=4$.}
    \label{fig:cifar-accumulation-1}
\end{figure}
\begin{figure}[p]
    \centering
    \includegraphics[width=\textwidth]{Experiments/new/cifar_comparison/cifar-averaging-comparison-2.pdf}
    \caption{Comparison of different $\alpha$ values using averaging scheme when training for CIFAR-10 dataset, using filter CGE with batch size 16, under fault type \textit{coordinate-wise}. Each row correspond to a different number of faults: (a) $f=1$, (b) $f=2$, (c) $f=3$, and (d) $f=4$.}
    \label{fig:cifar-accumulation-2}
\end{figure}

\subsubsection{Studies on combination of filters}

As is shown in the previous section, filters works well on some types of faults, while bad on others. We propose the method of combining different filters, in the hope that it will tolerate multiple types of faults.\\

First, we conducted experiments on \emph{mkrum}, where both multi-KRUM and CGE have difficulty converging. Multi-KRUM has a relatively high time complexity while CGE does not. By concatenating the two filters, we hope the performance would improve with little increase on time complexity. Results shown in Figure \ref{fig:experiment-results-4}, we observe that such concatenation does improve multi-KRUM (as well as CGE), that it is converging while neither of the two filters would not converge when applied alone. However, we also observe that by increasing the tolerance threshold, e.g. try to tolerate 20 fault when the real number is 10, multi-KRUM and CGE can have better performance too.

\begin{figure}[t]
    \centering
    \subcaptionbox{Loss}{
        \begin{minipage}{0.31\linewidth}
        \includegraphics[width=\linewidth]{Experiments/concatenation/loss-mnist-16-5-krum2-concat.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/concatenation/loss-mnist-16-10-krum2-concat.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/concatenation/loss-mnist-64-5-krum2-concat.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/concatenation/loss-mnist-64-10-krum2-concat.pdf}
        \end{minipage}
    }
    \subcaptionbox{Prec@1}{
        \begin{minipage}{0.31\linewidth}
        \includegraphics[width=\linewidth]{Experiments/concatenation/prec1-mnist-16-5-krum2-concat.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/concatenation/prec1-mnist-16-10-krum2-concat.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/concatenation/prec1-mnist-64-5-krum2-concat.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/concatenation/prec1-mnist-64-10-krum2-concat.pdf}
        \end{minipage}
    }
    \subcaptionbox{Prec@3}{
        \begin{minipage}{0.31\linewidth}
        \includegraphics[width=\linewidth]{Experiments/concatenation/prec3-mnist-16-5-krum2-concat.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/concatenation/prec3-mnist-16-10-krum2-concat.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/concatenation/prec3-mnist-64-5-krum2-concat.pdf}\vspace{-15pt}
        \includegraphics[width=\linewidth]{Experiments/concatenation/prec3-mnist-64-10-krum2-concat.pdf}
        \end{minipage}
    }
    \caption{Comparison between concatenated filters. Type of fault: \emph{mkrum}. Each row from left to right are (a) Loss, (b) Precision at 1, and (c) Precision at 3 on testing dataset of MNIST. Settings from top to bottom (batch-size and number of faults): (1) 16, 5, (2) 16, 10, (3) 64, 5, and (4) 64, 10.}
    \label{fig:experiment-results-4}
\end{figure}
\fi

==> experiments.tex <==
\section{Experiments}
\label{sec:exp}
In this section, we present our empirical studies on fault-tolerance in distributed learning of artificial neural networks using the D-SGD method and different gradient-filters, including our proposed CGE gradient-filter.
To evaluate the fault-tolerance of different gradient-filters we conduct experiments with different fractions of faulty agents $f/n$, different fault types, and different data batch-sizes $k$ used for computing stochastic gradients by non-faulty agents (see Section~\ref{sub:s_grad}).

\subsection{Implementation and setup}
\label{sub:implementation-and-setup}

We simulate the distributed server-based system architecture by spawning multiple threads, one for a server and others for the agents, where inter-thread communication is done through message passing interface (MPI). Our simulator is built in Python using PyTorch~\cite{paszke2017automatic} and MPI4py~\cite{dalcin2011parallel}, and is deployed on a Google Cloud Platform cluster made available by the Massive Data Institute at Georgetown University. The cluster we use has 64 vCPU cores and a memory of 100 GB.\\

% We implement our simulator for Byzantine fault-tolerant distributed machine learning system, partially based on the code from \cite{chen2018draco}. 
In our experiments, we consider distributed learning of artificial neural networks for supervised classification of two benchmark datasets; the MNIST dataset~\cite{lecun1998gradient} and the CIFAR-10 dataset~\cite{krizhevsky2009learning}. For all our experiments we consider the system to be synchronous and $n = 10$ agents. The server thread initiates the D-SGD method with the initial estimate $w^0$, a $d$-dimensional vector where the value of $d$ is equal to the total number of parameters of the artificial neural network being learned, using the initialization technique of Kaiming uniform\cite{he2015delving}. For each iteration, in step {\bf S2}, the step-size $\eta_t=0.1$ for all the gradient-filters described below.\\

In the subsequent sections, Section~\ref{sub:filters-descriptions} and Section~\ref{sub:fault-types}, we describe the other gradient-filters and the different types of faults, respectively.

\subsection{Other gradient-filters}
\label{sub:filters-descriptions}

Besides the CGE gradient-filter, we also evaluate fault-tolerance by four other state-of-the-art gradient-filters: geometric median, geometric median of means~\cite{chen2017distributed}, coordinate-wise trimmed mean~\cite{yin2018byzantine}, and multi-KRUM~\cite{blanchard2017machine}. Similar to the CGE gradient-filter, these other gradient-filters are implemented by the server in the second step, i.e., step {\bf S2}, of each iteration of the iterative algorithm described in Section~\ref{sub:steps}.\\

\begin{itemize}
\setlength\itemsep{0.5em}
    \item \textbf{Geometric median} (GeoMed): For a set of vectors $\{y_1,\ldots, \, y_n\}$ in $\R^d$, their geometric median denoted by $\mathsf{med}\{y_1,\ldots, \, y_n\}$ is defined to be
    \begin{align}
        \med\{y_1, \ldots, \, y_n\}=\arg\min_{y\in\mathbb{R}^d}\sum_{j=1}^n\norm{y_j-y}. \label{eqn:def_geomed}
    \end{align}
    The geometric median is less sensitive to outlying vectors than the arithmetic average~\cite{10.2307/2241834, mottonen2010asymptotic}.\\
    
    % Note that if the dimension of the vectors $y_i, i = 1, \ldots, \, n$ is equal to one then the geometric median is same as to the median statistics for scalar values. 
    % The geometric median is considered robust against outlying vectors  \\
    In GeoMed gradient-filter, in step {\bf S2} of each iteration $t$ the server computes the geometric median of the received stochastic gradients $\med\{g^t_1, \ldots, \,g^t_n\}$, and updates the current estimate $w^t$ to
    % Geometric median is widely used in robust statistics . This filter simply use the geometric median of all received gradients as vectors in Euclidean space to update the parameters, without considering how many faulty agents might be there. The geometric median of a set of vectors $\{y_1,...,y_n\}$, denoted by $\mathsf{med}\{y_1,...,y_n\}$, is defined as
    %     \[\med\{y_1,...,y_n\}=\arg\min_{y\in\mathbb{R}^d}\sum_{j=1}^n||g_j^t-y||_2\] 
    % where $d$ is the size of parameters $w^t$, hence also the size of any gradient $g^t_j$. The iterative process (\ref{eqn:algo_1}) changes as follows:
        \[w^{t+1}=w^t-\eta_t\cdot\med\{g^t_1, \ldots, \,g^t_n\}\]
    where $\eta_t$ denotes the step-size for iteration $t$. 
    \item \textbf{Geometric median of means} (MoM): For the MoM gradient-filter the server divides apriori the agents into $l$ groups indexed from $1$ to $l$. For simplicity, we assume that the total number of agents $n$ is a multiple of $l$. Thus, each group has $b = n/l$ agents. Let agents $\{1, \ldots, \, b\}$ belong to group $1$, agents $\{b+1, \ldots, \, 2b\}$ belong to group $2$, and so on. \\
    
    In step {\bf S2} of each iteration $t$, for each group $j \in \{1, \ldots, \, l\}$ the server computes the average $\widehat{g^t_j}$ of the stochastic gradients received from the agents in group $j$. Specifically, for each group $j \in \{1, \ldots, \, l\}$,
    \[\widehat{g^t_j}  = \frac{1}{b}\sum_{j=1}^bg^t_j.\]
    Then, the server computes the geometric median of all the groups' averaged stochastic gradients $\med\left\{\widehat{g^t_1}, \ldots, \,\widehat{g^t_n}\right\}$ as defined in~\eqref{eqn:def_geomed}. Finally, the server updates the current estimate $w^t$ to
        \[w^{t+1}=w^t-\eta_t\cdot\med\left\{\widehat{g^t_1}, \ldots, \,\widehat{g^t_n}\right\}.\]
        
    \item \textbf{Coordinate-wise trimmed mean} (CWTM): For a set of real scalar values $\{a_1,...,a_n\}$, with $a_1 \leq \ldots \leq a_n$, the $f$-trimmed mean denoted by $\mathsf{tm}_f\{a_1,...,a_n\}$ is defined to be
    \begin{align}
        \mathsf{tm}_f\{a_1, \ldots, \, a_n\} = \frac{1}{n-2f}\sum_{j = f+1}^{n-f}a_j. \label{eqn:def_tm}
    \end{align}
    
    The CWTM gradient-filter is an extension of the scalar trimmed mean filter which was proposed by Su and Vaidya~\cite{su2016fault}. In CWTM gradient-filter in each iteration the server updates its current estimate using a vector whose elements are $f$-trimmed means of the corresponding elements of the stochastic gradients received. Specifically, let the $l$-th element of a vector $y \in \R^d$ be denoted by $y[l]$. In step {\bf S2} of each iteration $t$, the server computes a vector $\widehat{g^t}$ such that for each $l=1,...,d$,
    \[\widehat{g^t}[l] = \mathsf{tm}_f\left\{g^t_1[l], \ldots, \, g^t_n[l] \right\}.\]
    Finally, the server updates the current estimate $w^t$ to
        \[w^{t+1}=w^t-\eta_t\cdot\widehat{g^t}.\]
    % emove the largest and smallest $f$ values in $\{g_1^t[k],...,g_n^t[k]\}$, then calculate the average of the rest values to obtain the $k$-th value of $\widehat{g^t}$. The iterative process (\ref{eqn:algo_1}) changes as follows:
    %     \[w^{t+1}=w^t-\eta_t\cdot\widehat{g^t}\]
        
    \item \textbf{Multi-KRUM}: In the multi-KRUM gradient-filter, in each iteration $t$ the server computes the {\em KRUM score} for each stochastic gradient received from the agents~\cite[Section 2]{blanchard2017machine}. The server chooses $m$ stochastic gradients with $m$ smallest KRUM scores and computes their average $g^t_{km}$. The parameter $m$ is chosen a priori such that $1\leq m\leq n-f$. The server updates the current estimate $w^t$ to
        \[w^{t+1}=w^t-\eta_t\cdot g^t_{km}.\]
    The value of $m$ chosen for our experiments is specified later. 
    % and update the parameters using $\widehat{g^t}$, the average of the gradients with the smallest $m$ KRUM scores, where $m$ ($1\leq m\leq n-f$) is a user-designated value, and calculating KRUM score also evolves $f$. The iterative process (\ref{eqn:algo_1}) changes as follows:
    %     \[w^{t+1}=w^t-\eta_t\cdot\widehat{g^t}\]
\end{itemize}

\subsection{Fault types}
\label{sub:fault-types}

Recall that Byzantine faulty agents can exhibit arbitrary faults. We conduct experiments for $5$ different types of faults, described below. In the first three fault types, the faulty agents are assumed Byzantine and omniscient. In the last two fault types, the faulty agents are assumed inadvertent. 

% We are interested in how performance of each filter changes when facing different kinds of faults. We design different types of faults that are potentially bad for filters, assuming faulty agents are able to gain unlimited information and collaborate. The designs are as follows, suppose the real number of faulty agents is $f'$:

\begin{itemize}
    \item \textbf{Gradient-reverse faults}: In this particular fault type, each faulty agent reverses its correct stochastic gradient and scales the reversed gradients by a factor of $100$. Specifically, for each iteration $t$ and each agent $j$, let $s_j^t$ denote agent $j$'s correct stochastic gradient for iteration $t$. If agent $j$ is faulty then it sends to the server an incorrect gradient
        \[g_j^t = -100\cdot s_j^t.\]
    %\item[\emph{medofmeans}] For median of means, the faulty gradients reverse the correct gradients and times 100, and faulty agents are distributed to as many groups in median of means as possible;
    \item \textbf{Coordinate-wise faults}: In this particular fault type, each fault agent sends a vector whose elements are equal to the $f$-th smallest respective elements of the stochastic gradients computed by the non-faulty agents. Specifically, if $\H$ denotes the set of all non-faulty (or honest) agents then for each faulty $j$ and $l \in \{1, \ldots, \, d\}$,
    \[g^t_j[l]=\text{the }f\text{-th smallest amongst }\left\{ g_i^t[l], ~ i\in \H \right\}, \quad \forall t.\]
    Recall that for a vector $y \in \R^d$, $y[l]$ denotes its $l$-th element.
    % in iteration $t$, each faulty agent $j$ sends a vector $g^t_j$ for its stochastic gradient such thatmakes the coordinate-wise $(f'+1$)th-smallest values among all honest agents the corresponding values for each coordinate in the faulty gradient. Let $l$-th element of a vector $y$ be denoted by $y[l]$. Instead of $g_k^t$, the vector $\widetilde{g_k^t}$ is send to the server by faulty agent $k$, where
    %\item[\emph{mkrum}] For multi-KRUM, the faulty gradients equal to the good gradient that has the largest KRUM score, i.e. the least possiblility of being chosen by KRUM algorithm, and
    \item \textbf{Norm-confusing faults}: In this particular fault type, each faulty agent reverses its correct stochastic gradient, and re-scales it so that its norm is equal to the $(f+1)$-th largest norm amongst the stochastic gradients computed by all the non-faulty agents. Specifically, for each iteration $t$, let $s^t_i$ denote a correct stochastic gradient for each agent $i$. Let, $\nu_t$ denote the non-faulty agent whose stochastic gradient's norm is $(f+1)$-th largest amongst the norms of all the non-faulty agents' stochastic gradients. Then each faulty agent $j$ sends to the server an incorrect stochastic gradient
    \[g^t_j = - \left(\frac{\norm{g^t_{\nu_t}}}{\norm{s^t_j}}\right) \cdot s^t_j, \quad \forall t. \]
        % $$\widetilde{g_k^t}=-n_{f'+1}\cdot g_k^t$$
    %\item \textit{normfilter-collaborative}: \shuo{suggestion 1} A faulty agent averages the honest gradients, reverses it, and has the $(f'+1)$th-largest norm among all honest agents. Let $n_{f'+1}$ be the $(f'+1)$th-largest norm among honest agents. Instead of $g_k^t$, the following vector is send to the server by faulty agent $k$:
    %    $$\widetilde{g_k^t}=-n_{f'+1}\cdot\frac{1}{|H|}\sum_{j\in H}g_j^t$$
    %\item \textit{omniscient}\cite{xie2018generalized}: \shuo{suggestion 2} A faulty agent averages the honest gradients, reverses it, and times a large constant (1e20). Let $n_{f'+1}$ be the $(f'+1)$th-largest norm among honest agents. Instead of $g_k^t$, the following vector is send to the server by faulty agent $k$:
    %    $$\widetilde{g_k^t}=-10^{20}\cdot\frac{1}{|H|}\sum_{j\in H}g_j^t$$
\end{itemize}

We also conduct experiments for a few non-Byzantine inadvertent fault types described below. These faults are known to occur in practice due to system hardware failures~\cite{xie2018generalized, he2020byzantinerobust}.

\begin{itemize}
    \item \textbf{Label-flipping faults}: In this particular fault type, a faulty agent sends incorrect stochastic gradients due to the output classification labels of their sampled data points being erroneous. To simulate this fault in the case of MNIST or CIFAR-10 data-sets, where there are 10 differnet labels in each of them, for each data point sampled by a faulty agent, we change the original label of the data point $y$ to $\widetilde{y}=9-y$.
    %\item \textit{bitflipping}: A faulty agent sends bad gradients because the sign bits are corrupted due to hardware failure. In stead of $g_k^t$, the following vector is send to server by faulty agent $k$:
    %    $$\widetilde{g_k^t}=-g_k^t$$
    \item \textbf{Random faults}: As the name suggests, in this particular fault type, each faulty agent sends a randomly chosen vector from $\R^d$ for its stochastic gradient to the server in each iteration. In our experiments, we consider a scenario where the faulty agents send i.i.d.~Gaussian random vectors of mean $0$ and an isotropic covariance matrix with standard deviation of $200$.
\end{itemize}

% simulate the D-SGD method we consider The server thread simulates the We consider a system architecture of $n = 10$ agentsthe distributed optimization of neural network is done in server-based model, where in each step, server send current parameters to agents, multiple agents then calculate gradients and send them to the server, server after filtering the gradients it receives, updates the parameters, and sends the parameters back to all agents, as we have discussed in Section \ref{sec:intro}. \\

% Next, we present the remaining details and outcomes of our experiments.

\subsection{Results and analysis}

As mentioned above, we consider supervised learning of artificial neural networks for classifying images in two different data-sets; MNIST and CIFAR-10. First, we will present our results for the MNIST dataset below.

\subsubsection{MNIST Dataset}
\label{subsub:mnist}

MNIST is an image-classification dataset of handwritten digits comprising $60,000$ training samples and $10,000$ testing samples~\cite{lecun1998gradient}. We consider a convolutional neural network called $\mathsf{LeNet}$ for the classification task that comprises of $431,080$ learning parameters. Thus, the value of dimension $d = 431,080$. \\

The outcomes for our different experiments are presented below.\\

{\bf Different fault types:} To compare the performance of different gradient-filters under the different types of faults described above in Section~\ref{sub:fault-types}, 
\begin{itemize}
    \item we fix the data batch-size used for computing stochastic gradients by all the non-faulty agents to $k = 16$ (see Section~\ref{sub:s_grad}), and 
    \item we consider just $1$ faulty agent in the system, i.e., $f = 1$, out of $n = 10$ total agents. Without loss of generality we let agent $1$ to be the faulty agent. Note that the identity of the faulty agent is hidden from other non-faulty agents and the server.
\end{itemize}

The plots in Figure~\ref{fig:fault-types-1} show the learning curve for the different Byzantine faults, while the plots in Figure~\ref{fig:fault-types-2} show the learning curve for the different inadvertent faults. \\

As is shown in the figures, since the fraction of faulty agents is small here, the D-SGD method converges for all five gradient-filters. We also observe that, unlike the other gradient-filters, the fault-tolerance by CGE gradient-filter is consistently good for all the different types of faults. However, note that in the case of \textit{coordinate-wise faults} shown in Figure~\ref{fig:fault-types-1}(b), the learning curve for all the gradient-filters is quite erratic. There are large `spikes' in the loss plots, and corresponding `dives' in the precision plots. \\
% while only multi-KRUM behaves relatively stable, as is shown in Figure~\ref{fig:fault-types-1}(b). 
% Moreover, these We observe that actually small `pikes' also shows in fault-free plot near the same steps. 
% One possible reason for this phenomenon is that coordinate-wise constructed faults cannot be easily addressed by most of the filters, while the only coordinate-wise filter we have are even more specifically targeted. As a result, the faulty gradients are likely not to be filtered out. \\

% We observe that multi-KRUM has the worst performance, that SGD tends to converge to a loss value farther from the `correct' value than when applying other filters, under all types of faults. Considering the cluster-based technique this filter applies, it is likely that high variance of good gradients in each step, which is a result of small batch size, makes multi-KRUM hard to find faulty gradients. \\

\begin{figure*}[htb!]
    \centering
    \includegraphics[width=\textwidth]{Experiments/new/fault_types_comparison/fault-type-comparison-1.pdf}
    \caption{Distributed learning of neural networks for MNIST dataset using the D-SGD method and the different gradient-filters as mentioned in presence of $f = 1$ faulty agent exhibiting the different Byzantine faults. Each row corresponds to a different fault type: (a) \textit{gradient reverse}, (b) \textit{coordinate-wise}, and (c) \textit{norm-confusing}. The first column plots the training loss, whilst the second column plots the testing precision, versus the number of iterations or steps.}
    \label{fig:fault-types-1}
\end{figure*}

\begin{figure*}[htb!]
    \centering
    \includegraphics[width=\textwidth]{Experiments/new/fault_types_comparison/fault-type-comparison-2.pdf}
    \caption{Distributed learning of neural networks for MNIST dataset using the D-SGD method and the different gradient-filters as mentioned in presence of $f = 1$ faulty agent exhibiting the different inadvertent faults. Each row corresponds to a different type of fault: (a) \textit{label-flipping} and (b) \textit{random}. The two columns plot the training loss and the testing precision, respectively.}
    \label{fig:fault-types-2}
\end{figure*}

{\bf Different data batch-sizes:}
To evaluate the influence of individual agents' data batch-sizes, i.e., the value of $k$ in Section~\ref{sub:s_grad}, on fault-tolerance by a gradient-filter, we simulate the multi-KRUM and CGE gradient-filters for two different data batch-sizes: $k = 16$ and $k = 64$. The learning curves for the two filters for two different Byzantine fault types, namely the {\em gradient reverse faults} and the {\em norm-confusing faults}, are shown in Figures~\ref{fig:batch-size-3},~\ref{fig:batch-size-4},~\ref{fig:batch-size-5} and~\ref{fig:batch-size-6}. In all these figures we plot the loss and precision upon the completion of the $100$-th step or iteration.\\

Upon comparing the plots in the aforementioned figures we observe that the fault-tolerance of both multi-KRUM and CGE gradient-filter improves significantly with increase in the data batch-size. This is indeed coherent with the theoretical analysis of CGE gradient-filter presented in Section~\ref{sub:ft}. Intuitively, a higher batch-size results in stochastic gradients with improved accuracy and reduced noise or variance. Thus, it is only reasonable for gradient-filters to achieve better fault-tolerance when non-faulty agents compute stochastic gradients by sampling a larger number of data points in each iteration. However, this improvement is accompanied by an increased cost for computation of stochastic gradients in each iteration. \\


% mentio~\ref{fig:batch-size-3} and Figure~\ref{fig:batch-size-4}, we note that multi-KRUM works generally handles \textit{reverse} and \textit{norm-confusing} with a similar capability, while it becomes more difficult when number of faulty agents is larger under \textit{norm-confusing}. There is a significant improvement under both fault types when batch size increases from 16 to 64. With batch size being 64, it is with higher probability that good agents, drawn with identical independent distribution, would return a group of gradients with lower variance in a step. This also confirms our proposition in the previous subsection, that multi-KRUM works better when the variance of good gradients are lower.\\

% Similarly, comparing Figure~\ref{fig:batch-size-4} and Figure~\ref{fig:batch-size-5}, we see that CGE handles \textit{reverse} better than \textit{norm-confusing}, which is understandable since \textit{reverse} provides faults that are more distinguishable to CGE. Meanwhile, we don't see a similar instability of multi-KRUM when facing more faulty agents under \textit{norm-confusing}, that batch size does not effect performance of CGE significantly. \\

\begin{figure*}[p]
    \centering
    \includegraphics[width=\textwidth]{Experiments/new/batch_size_comparison/batch-size-comparison-3.pdf}
    \caption{Distributed learning of neural networks for MNIST dataset using the D-SGD method and the multi-KRUM gradient-filter ($m = 2$) with different data batch-sizes. The faulty agents exhibit the \textit{gradient reverse} faults. Different rows present the cases with different number of faults $f$; (a) $f=1$, (b) $f=2$, (c) $f=3$, and (d) $f=4$. The two columns plot the training loss and testing precision, respectively.}
    \label{fig:batch-size-3}
\end{figure*}
\begin{figure*}[p]
    \centering
    \includegraphics[width=\textwidth]{Experiments/new/batch_size_comparison/batch-size-comparison-4.pdf}
    \caption{Distributed learning of neural networks for MNIST dataset using the D-SGD method and the multi-KRUM gradient-filter ($m = 2$) with different data batch-sizes. The faulty agents exhibit the \textit{non-confusing} faults. Different rows present the cases with different number of faults $f$; (a) $f=1$, (b) $f=2$, (c) $f=3$, and (d) $f=4$. The two columns plot the training loss and testing precision, respectively.}
    \label{fig:batch-size-4}
\end{figure*}
\begin{figure*}[p]
    \centering
    \includegraphics[width=\textwidth]{Experiments/new/batch_size_comparison/batch-size-comparison-5.pdf}
    \caption{Distributed learning of neural networks for MNIST dataset using the D-SGD method and the CGE gradient-filter with different data batch-sizes. The faulty agents exhibit the \textit{gradient reverse} faults. Different rows present the cases with different number of faults $f$; (a) $f=1$, (b) $f=2$, (c) $f=3$, and (d) $f=4$. The two columns plot the training loss and testing precision, respectively.}
    \label{fig:batch-size-5}
\end{figure*}
\begin{figure*}[p]
    \centering
    \includegraphics[width=\textwidth]{Experiments/new/batch_size_comparison/batch-size-comparison-6.pdf}
    \caption{Distributed learning of neural networks for MNIST dataset using the D-SGD method and the CGE gradient-filter with different data batch-sizes. The faulty agents exhibit the \textit{norm-confusing} faults. Different rows present the cases with different number of faults $f$; (a) $f=1$, (b) $f=2$, (c) $f=3$, and (d) $f=4$. The two columns plot the training loss and testing precision, respectively.}
    \label{fig:batch-size-6}
\end{figure*}

{\bf Different fractions of faulty agents:}
% \label{ssub:frac-of-faults}
We evaluate the fault-tolerance of mult-KRUM and CGE gradient-filters in the presence of varied fraction of faulty agents, with different faulty behaviors. The plots are shown in Figures~\ref{fig:fault-fraction-1} to \ref{fig:fault-fraction-4}. As expected, the learning process for both the gradient-filters deteriorates with increase in the fraction of faults. \\

From the plots in the aforementioned figures, we observe that whilst the increase in $f/n$ has adversarial effects on the fault-tolerance, the increase in the batch-size improves the fault-tolerance for any given fraction of faults. At large, the observed effects on the fault-tolerance achieved by the CGE gradient-filter to change in the fraction of faults $f/n$ is coherent with the theoretical analysis presented in Section~\ref{sub:ft}.\\

Next, we present experimental results for the case of CIFAR-10 dataset.

% When fraction of faulty agents is larger or equal to 50\%, the fault-tolerant task become meaningless. For comparison purpose, we also document a group of results for reference, where no gradient filter is applied, that only plain averaging is used upon receiving gradients from agents, in Appendix \ref{sub:exp-with-no-filter}. \\

% It is shown in the Figures that CGE is generally more stable than multi-KRUM, that in most cases, SGD would converge rapidly and to a value that is close to the fault-free convergence, while multi-KRUM might take more steps, and there might be a gap between the value SGD converges to and the value of fault-free convergence. Notice that when batch size increases such gap is become smaller, but as is shown by plots in Figure~\ref{fig:fault-fraction-4}, the gap still exists when batch size is larger.\\

% One thing worth noticing, which is also observed in previous experiments, is that SGD under both filters shows the unstable behavior we have seen previously, under \textit{coordinate-wise} type of fault, regardless of batch size, but only when the number of faulty agents is 1 or 2. When the fraction of faulty agents become larger, the training loss become stable instead. Notice that under \textit{coordinate-wise} fault, faulty agents produce their bad gradients collaboratively but everyone of them produces the same bad gradient in each step; which might be the reason since the bad gradients become easier for filters to spot when there are more of them.

\begin{figure*}[p]
    \centering
    \includegraphics[width=\textwidth]{Experiments/new/fault_fraction_comparison/num-faults-comparison-1.pdf}
    \caption{Distributed learning of neural networks for MNIST dataset using the D-SGD method and the CGE gradient-filter under different number of faulty agents $f$ out of $n = 10$. In these experiments the data batch-size $k = 16$. Different rows present different fault types: (a) \textit{gadient reverse}, (b) \textit{coordinate-wise}, (c) \textit{norm-confusing}, (d) \textit{label-flipping}, and (e) \textit{random}. The two columns plot the training loss and the testing precision, respectively.}
    \label{fig:fault-fraction-1}
\end{figure*}
\begin{figure*}[p]
    \centering
    \includegraphics[width=\textwidth]{Experiments/new/fault_fraction_comparison/num-faults-comparison-2.pdf}
    \caption{Distributed learning of neural networks for MNIST dataset using the D-SGD method and the multi-KRUM ($m=2$) gradient-filter under different number of faulty agents $f$ out of $n = 10$. In these experiments the data batch-size $k = 16$. Different rows present different fault types: (a) \textit{gadient reverse}, (b) \textit{coordinate-wise}, (c) \textit{norm-confusing}, (d) \textit{label-flipping}, and (e) \textit{random}. The two columns plot the training loss and the testing precision, respectively.}
    \label{fig:fault-fraction-2}
\end{figure*}
\begin{figure*}[p]
    \centering
    \includegraphics[width=\textwidth]{Experiments/new/fault_fraction_comparison/num-faults-comparison-3.pdf}
    \caption{Distributed learning of neural networks for MNIST dataset using the D-SGD method and the CGE gradient-filter under different number of faulty agents $f$ out of $n = 10$. In these experiments the data batch-size $k = 64$. Different rows present different fault types: (a) \textit{gadient reverse}, (b) \textit{coordinate-wise}, (c) \textit{norm-confusing}, (d) \textit{label-flipping}, and (e) \textit{random}. The two columns plot the training loss and the testing precision, respectively.}
    \label{fig:fault-fraction-3}
\end{figure*}
\begin{figure*}[p]
    \centering
    \includegraphics[width=\textwidth]{Experiments/new/fault_fraction_comparison/num-faults-comparison-4.pdf}
    \caption{Distributed learning of neural networks for MNIST dataset using the D-SGD method and the multi-KRUM ($m=2$) gradient-filter under different number of faulty agents $f$ out of $n = 10$. In these experiments the data batch-size $k = 64$. Different rows present different fault types: (a) \textit{gadient reverse}, (b) \textit{coordinate-wise}, (c) \textit{norm-confusing}, (d) \textit{label-flipping}, and (e) \textit{random}. The two columns plot the training loss and the testing precision, respectively.}
    \label{fig:fault-fraction-4}
\end{figure*}

\newpage
\subsubsection{CIFAR-10 Dataset}
\label{subsub:cifar}

Similar to MNIST dataset, CIFAR-10 is also an image-classification dataset comprising $60,000$ small color images in $10$ mutually exclusive categories, \emph{e.g.} automobile, bird, dog, etc., with equal number of images in each class~\cite{krizhevsky2009learning}. The CIFAR dataset is further divided into $50,000$ training samples and $10,000$ testing samples. Classification in CIFAR-10 is expected to be more difficult than MNIST, since the images in MNIST are monochromatic and has less variety. On the other hand, the images in CIFAR-10 are quite diverse. For instance, an image of a sedan and a SUV both belong to the class of automobiles, and different breeds of dogs can look very differently from each other. Similar to MNIST, we again consider the convolutional neural network $\mathsf{LeNet}$ with $657,080$ learning parameters. Thus, the value of dimension $d = 657,080$ in this particular case. The experimental results are shown in Figure~\ref{fig:cifar-1} with specific details provided in the captions.\\

Next, we present a {\em gradient averaging} scheme that aims to reduce the sensitivity of fault-tolerance achieved by a gradient-filter to individual agents' data batch-size $k$.

% We use the same class of convolutional neural networks $\mathsf{LeNet}$, as for the MNIST dataset above, and perform similar experiments. 


% Some of the results are documented here in Figure~\ref{fig:cifar-1}. As CIFAR-10 is a more difficult task to MNIST and we are using the same neural network, we see that the speed of convergence is much slower than what we have in MNIST, and with the same 300 steps, we can only see a trend of convergence. But still, some filters works better than others. Geometric median (a), median of means (b), and coordinate-wise trimmed mean (c) cannot handle the case where there are 4 out of 10 fault agents. There is a gap between multi-KRUM plots and fault-free plot, while CGE, out of the five filters, help SGD converge with a speed close to the fault-free case. The relative performance of filters are basically the same as in MNIST, that CGE works generally better than mutli-KRUM no matter which dataset is using.\\

\begin{figure*}[p]
    \centering
    \includegraphics[width=\textwidth]{Experiments/new/cifar_comparison/cifar-filter-comparison-1.pdf}
    \caption{Distributed learning of neural networks for CIFAR-10 dataset using the D-SGD method and the different gradient-filters in presence of $f = 1$ faulty agent, out of $n=10$ total agents, exhibiting the \textit{coordinate-wise} faults. In these experiments the data batch-size $k = 16$. Different rows correspond to different gradient-filters: (a) geometric median, (b) median of means, (c) coordinate-wise trimmed mean, (d) multi-KRUM with $m=2$, and (e) CGE.}
    \label{fig:cifar-1}
\end{figure*}




==> experiments_aaai.tex <==
\section{Experiments}
\label{sec:exp}

In this section, we present our key empirical results on fault-tolerance in distributed learning of artificial neural networks using the D-SGD method in conjunction with different gradient-filters. We consider two benchmark image classification tasks; MNIST~\cite{lecun1998gradient} and CIFAR-10~\cite{krizhevsky2009learning}. The fault-tolerance of different gradient-filter is evaluated through multiple experiments with varied fractions of faulty agents $f/n$, different types of faults and the data batch-size $k$.\\

% \subsection{Implementation and setup}
% \label{sub:implementation-and-setup}

{\bf Setup:} To simulate the distributed server-based system architecture (shown in Figure~\ref{fig:algo}) we spawn multiple threads, one for a server and others for the agents. The inter-thread communication is done through message passing interface (MPI). The simulator is built in Python using PyTorch~\cite{paszke2019pytorch} and MPI4py~\cite{dalcin2011parallel}, and is deployed on a Google Cloud Platform cluster% made available by the Massive Data Institute at Georgetown University
. The cluster we use has 64 vCPU cores and a memory of 100 GB.\\

We simulate a distributed system with $n = 40$ agents, and $f$ faulty agents that are chosen randomly. The server initiates the D-SGD method by choosing the initial estimate $w^0$ by uniform distributions near 0, a $d$-dimensional vector where $d$ is the total number of parameters of the artificial neural network used whose details are presented shortly. The step-size $\eta_t=0.01$ in all iterations. To tolerate faulty agents, the server uses a gradient-filter as shown in step S2 of Algorithm~\ref{alg:cge}. We compare the fault-tolerance of our CGE gradient-filter with the following prominent gradient-filters.
\begin{itemize}
    \item Geometric median (GeoMed);
    \item Geometric median-of-means (MoM)~\cite{chen2017distributed}, with group size $b = 2$;
    \item Coordinate-wise trimmed mean (CWTM)~\cite{yin2018byzantine};
    \item Multi-KRUM~\cite{blanchard2017machine}, with $m = 5$.
\end{itemize}
~

{\bf Types of Faults:} We simulate faulty agents that can exhibit two different types of faults listed below. The second one simulates inadvertently faulty agents that exhibit faulty behaviors due to hardware failures~\cite{he2020byzantinerobust}. 

% {\bf Other gradient-filters:} We compare the fault-tolerance of our CGE gradient-filter with the following three state-of-the-art gradient-filters. 

% Similar to Algorithm~\ref{alg:cge}, all 
% geometric median of means~\cite{chen2017distributed}, coordinate-wise trimmed mean~\cite{yin2018byzantine}, and . Similar to the CGE gradient-filter, these other gradient-filters are implemented by the server in the second step, i.e., step {\bf S2}, of each iteration of the iterative algorithm described in Section~\ref{sec:algo}.\\

% In our experiments, we use the following parameters: In median of means, agents are divided into groups to calculate means, where we choose group size $b=2$. In multi-KRUM, $m$ gradients with $m$ smallest KRUM scores are used to calculate update, where we choose $m=5$.
% Besides CGE

% The other gradient-filters we evaluate are briefly described as follows.\\

% % We implement our simulator for Byzantine fault-tolerant distributed machine learning system, partially based on the code from \cite{chen2018draco}. 
% % As mentioned above, we consider distributed learning of artificial neural networks for MNIST and CIFAR-10. For the experiments, we assume the system to be synchronous and $n = 40$ agents. 

% % In the subsequent sections, Section~\ref{sub:filters-descriptions} and Section~\ref{sub:fault-types}, we describe the other gradient-filters and the different types of faults, respectively.

% \subsection{Other gradient-filters}
% \label{sub:filters-descriptions}

% \subsection{Fault types}
% \label{sub:fault-types}

% We evaluate the fault-tolerance of the above gradient-filters and CGE under $4$ different types of faults simulated by the Byzantine faulty agents. , described below. 


% We are interested in how performance of each filter changes when facing different kinds of faults. We design different types of faults that are potentially bad for filters, assuming faulty agents are able to gain unlimited information and collaborate. The designs are as follows, suppose the real number of faulty agents is $f'$:

\begin{itemize}
    \item \textbf{Gradient-reverse fault}: A faulty agent sends to the server a vector directed opposite to its correct stochastic gradient, but with the same norm. Specifically, if $s^t_i$ denotes a correct stochastic gradient of faulty agent $i$ in iteration $t$ then agent $i$ sends to the server a vector $g^t_i = - s^t_i$. %and scales the reversed gradients by a factor of $100$.~\cite{chen2018draco}
    %\item[\emph{medofmeans}] For median of means, the faulty gradients reverse the correct gradients and times 100, and faulty agents are distributed to as many groups in median of means as possible;
    %\item \textbf{Coordinate-wise faults}: Each faulty agent sends a vector whose elements are equal to the $f$-th smallest respective elements of the stochastic gradients computed by the non-faulty agents. Specifically, if $\H$ denotes the set of all non-faulty (or honest) agents then for each faulty $j$ and $l \in \{1, \ldots, \, d\}$,
    %\[g^t_j[l]=\text{the }f\text{-th smallest amongst }\left\{ g_i^t[l], ~ i\in \H \right\}, \quad \forall t.\]
    %Recall that for a vector $y \in \R^d$, $y[l]$ denotes its $l$-th element.
    % in iteration $t$, each faulty agent $j$ sends a vector $g^t_j$ for its stochastic gradient such thatmakes the coordinate-wise $(f'+1$)th-smallest values among all honest agents the corresponding values for each coordinate in the faulty gradient. Let $l$-th element of a vector $y$ be denoted by $y[l]$. Instead of $g_k^t$, the vector $\widetilde{g_k^t}$ is send to the server by faulty agent $k$, where
    %\item[\emph{mkrum}] For multi-KRUM, the faulty gradients equal to the good gradient that has the largest KRUM score, i.e. the least possiblility of being chosen by KRUM algorithm, and
    %%\item \textbf{Norm-confusing fault}: Similar to gradient-reverse fault, a faulty agent sends to the server a vector directed opposite to its correct stochastic gradient. However, in this particular type of fault, the norm of the vector is equal to the $(f+1)$-th largest norm amongst the stochastic gradients computed by all the $n-f$ non-faulty agents. 
        % $$\widetilde{g_k^t}=-n_{f'+1}\cdot g_k^t$$
    %\item \textit{normfilter-collaborative}: \shuo{suggestion 1} A faulty agent averages the honest gradients, reverses it, and has the $(f'+1)$th-largest norm among all honest agents. Let $n_{f'+1}$ be the $(f'+1)$th-largest norm among honest agents. Instead of $g_k^t$, the following vector is send to the server by faulty agent $k$:
    %    $$\widetilde{g_k^t}=-n_{f'+1}\cdot\frac{1}{|H|}\sum_{j\in H}g_j^t$$
    %\item \textit{omniscient}\cite{xie2018generalized}: \shuo{suggestion 2} A faulty agent averages the honest gradients, reverses it, and times a large constant (1e20). Let $n_{f'+1}$ be the $(f'+1)$th-largest norm among honest agents. Instead of $g_k^t$, the following vector is send to the server by faulty agent $k$:
    %    $$\widetilde{g_k^t}=-10^{20}\cdot\frac{1}{|H|}\sum_{j\in H}g_j^t$$
%\end{itemize}

%We also conduct experiments for a few non-Byzantine inadvertent fault types described below. These faults are known to occur in practice due to system hardware failures~\cite{xie2018generalized, he2020byzantinerobust}.

%\begin{itemize}
    \item \textbf{Label-flipping fault}: A faulty agent sends incorrect stochastic gradients due to erroneous output classification labels of their data points.
    % output  of their sampled data points being erroneous. 
    Specifically, in our experiments where there are 10 different labels in both MNIST and CIFAR-10 data-sets, the original label of a data point $y$ sampled by a faulty agent is changed to $\widetilde{y}=9-y$.
    %\item \textit{bitflipping}: A faulty agent sends bad gradients because the sign bits are corrupted due to hardware failure. In stead of $g_k^t$, the following vector is send to server by faulty agent $k$:
    %    $$\widetilde{g_k^t}=-g_k^t$$
    %\item \textbf{Random fault}: A faulty agent sends a randomly chosen vector from $\R^d$ for its stochastic gradient to the server in each iteration. Specifically, in our experiments, a faulty agents sends i.i.d.~Gaussian random vectors with elements of mean value $0$ and standard deviation of $200$.
\end{itemize}

% simulate the D-SGD method we consider The server thread simulates the We consider a system architecture of $n = 10$ agentsthe distributed optimization of neural network is done in server-based model, where in each step, server send current parameters to agents, multiple agents then calculate gradients and send them to the server, server after filtering the gradients it receives, updates the parameters, and sends the parameters back to all agents, as we have discussed in Section \ref{sec:intro}. \\

% Next, we present the remaining details and outcomes of our experiments.
% Now, we present below our experimental results.

\subsection{Results and analysis}

We now present our experimental results with the above setup under various settings specified below. %Additional results are provided in the supplementary material for review purposes.  
% As mentioned above, we consider supervised distributed learning of artificial neural networks for classifying images in two different data-sets; MNIST and CIFAR-10. We have completed experiments in various settings, but due to limited space, we present some of them in this paper, whilst other results can be found in supplementary materials. 
First, we present our results for the MNIST image classification task~\cite{lecun1998gradient}.\\

% \subsubsection{MNIST Dataset}
% \label{subsub:mnist}

{\bf MNIST:} This is an image-classification dataset of handwritten digits comprising $60,000$ training samples and $10,000$ testing samples. For this particular classification task, we consider a state-of-the-art convolutional neural network $\mathsf{LeNet}$ that constitutes of $431,080$ learning parameters. Thus, in this case the value of dimension $d = 431,080$. \\

\begin{figure}[tb!]
    \centering
    \includegraphics[width=\linewidth]{Experiments/aaai/fault_type_comparison/fault-type-comparison-7.pdf}
    \caption{\footnotesize{\it Distributed learning of the convolutional neural network $\mathsf{LeNet}$ for the MNIST dataset using the D-SGD method with different gradient-filters (represented by different colors) to tolerate $f = 8$ faulty agents in the system. The training losses and the testing accuracies evaluated by the server after $0$ to $500$ iterations (or steps) of the different learning algorithms are plotted in the first and the second rows, respectively. Different columns contain the results for different types of faults simulated by the faulty agents. Here, the data batch size $k=64$.}}
    \label{fig:fault-types-03}
\end{figure}

% The outcomes for our different experiments are presented below.\\
We fix the number of faulty agents $f = 8$ out of $n = 40$ total agents, and the data batch-size $k = 64$. We do multiple experimental runs of the D-SGD method with different gradient-filters under different types of faults. The identity of the faulty agents is fixed across all the experiments. We also fix the random seed used by the agents for sampling their data points in the training phase, so that across different experiments the same agent samples the same mini-batch of data for the same iteration (or step). From our experiments, we observe that other than median-of-means, the three gradient-filters, including CGE, have comparable fault-tolerance against all the four types of faults exhibited by the faulty agents. Median-of-means cannot tolerate \emph{gradient-reverse} faults, and exhibits a performance gap between other filters when facing \emph{label-flipping} faults. The plots for the losses and accuracies versus the number of iterations (or steps) are shown in Figure~\ref{fig:fault-types-03} for the different experiments. Table~\ref{tab:run-time} shows the running time for each filter under \emph{label-flipping} faults. CGE has significantly smaller running time while preserving comparable performance.\\
%We have observed that the \textit{norm-confusing} faults pose a greater challenge to the CGE gradient-filter than the other three types of faults. \\

\begin{table}[tb!]
    \centering
    \caption{\footnotesize{Running time for distributed learning of \textsf{LeNet} for MNIST using D-SGD method with batch size $k=64$ and the different gradient-filters in presence of $f=8$ faulty agents exhibiting \emph{label-flipping} type of fault, corresponding to the training process shown in Fig.~\ref{fig:fault-types-03}(b). Total running time refers to the time for 500 iterations.}}
    \footnotesize
    \begin{tabular}{c|cc}
        \textbf{Filter} & \textbf{Time per iteration} (s) & \textbf{Total running time} (s) \\
        \hline
        GeoMed & 2.473 & 1236.5 \\
        MoM & 1.150 & 575.1 \\
        CWTM & 0.903 & 451.8 \\
        Multi-KRUM & 2.225 & 1112.4 \\
        CGE & \textbf{0.573} & \textbf{286.3} \\
    \end{tabular}
\label{tab:run-time}
\end{table}

\begin{figure}[tb!]
    \centering
    %\includegraphics[width=\linewidth, height = 0.45\linewidth]{Experiments/aaai/batch_size_comparison/batch-size-comparison-4.pdf}
    \includegraphics[width=\linewidth]{Experiments/aaai/batch_size_comparison/batch-size-comparison-5.pdf}
    \caption{\footnotesize{\it Average training losses and testing accuracies evaluated between $475$ to $500$ steps of the D-SGD method with CGE gradient-filter for distributed learning of the neural network $\mathsf{LeNet}$ (for the MNIST dataset) in the presence of different number of faulty agents $f$ (represented by different colors) each exhibiting the \emph{gradient-reverse} Byzantine fault, for different data batch-sizes.}}
    \label{fig:batch-size-01}
\end{figure}

% {\bf Different data batch-sizes:}
To evaluate the influence of individual agents' data batch-sizes on the fault-tolerance by CGE gradient-filter we conduct experiments with four different data batch-sizes: $k = 32, \, 64, \, 128$, and $256$. For these experiments all the faulty agents exhibit the {\em label-flipping} faults. The average training losses and testing accuracies between the $475$-th to $500$-th iterations (or steps) for different batch-sizes are shown in Figure~\ref{fig:batch-size-01} where different colors represent different numbers of faulty agents $f$. A larger data batch-size results in stochastic gradients with smaller variances (see~\eqref{eqn:avg_grad} in Section~\ref{sec:algo}), and thus, as expected from our theoretical results in Section~\ref{sec:ft}, the fault-tolerance of CGE gradient-filter improves with increase in the batch-size. However, an increase in the data batch-sizes proportionally increases the costs for computing the stochastic gradients in each iteration. We later present a {\em exponential averaging} technique that reduces the variances of the stochastic gradients, and improves the fault-tolerance of the CGE gradient-filter, without increasing the data batch-sizes or the costs for computing the stochastic gradients.\\

% it is only reasonable for a gradient-filter such as CGE to achieve better fault-tolerance when non-faulty agents compute stochastic gradients by sampling a larger number of data points in each iteration.\\

% As  the fault-tolerance of CGE gradient-filter improves with increase in the batch-size. 
%  
%  \\


% {\bf Different fault types:} To compare the performance of different gradient-filters under the different types of faults described above in Section~\ref{sub:fault-types}, 
% \begin{itemize}
%     \item we fix the data batch-size $k$ used for computing stochastic gradients by all the non-faulty agents to 64, and 
%     \item we consider $4$ faulty agent in the system, i.e., $f = 4$, out of $n = 40$ total agents. Note that the identity of the faulty agent is hidden from other non-faulty agents and the server.
%     \item 
% \end{itemize}



% As is shown in the figures, since the fraction of faulty agents is small here, the D-SGD method converges for all five gradient-filters. We also observe that, unlike the other gradient-filters, the fault-tolerance by CGE gradient-filter is consistently good for all the different types of faults. \\
% while only multi-KRUM behaves relatively stable, as is shown in Figure~\ref{fig:fault-types-1}(b). 
% Moreover, these We observe that actually small `pikes' also shows in fault-free plot near the same steps. 
% One possible reason for this phenomenon is that coordinate-wise constructed faults cannot be easily addressed by most of the filters, while the only coordinate-wise filter we have are even more specifically targeted. As a result, the faulty gradients are likely not to be filtered out. \\

% We observe that multi-KRUM has the worst performance, that SGD tends to converge to a loss value farther from the `correct' value than when applying other filters, under all types of faults. Considering the cluster-based technique this filter applies, it is likely that high variance of good gradients in each step, which is a result of small batch size, makes multi-KRUM hard to find faulty gradients. \\

\begin{figure}[tb!]
    \centering
    \includegraphics[width=\linewidth]{Experiments/aaai/num_faults_comparison/num-faults-comparison-4.pdf}
    \caption{\footnotesize{\it Average training losses and testing accuracies evaluated between $475$ to $500$ steps of the D-SGD method with CGE gradient-filter for distributed learning of the neural network $\mathsf{LeNet}$ (for the MNIST dataset) in the presence of varied number of faulty agents $f$. Different colors represent different types of faults. The data batch-size $k=64$. }}
    \label{fig:num-faults-01}
\end{figure}

% {\bf Different fractions of faulty agents:}
% \label{ssub:frac-of-faults}
Lastly, to evaluate the effect of increase in the fraction of faulty agents $f/n$ on the fault-tolerance of CGE gradient-filter we conduct experiments for different values of $f$. In these experiments we assume the data batch-size $k = 64$. The trend of average losses and accuracies observed between the $475$-th to $500$-th iterations (or steps) is shown in Figure~\ref{fig:num-faults-01}. As expected from our theoretical results in Section~\ref{sec:ft}, the fault-tolerance of the CGE gradient-filter deteriorates with increase in the fraction of faulty agents.\\

% From the above experimental results, it observe that whilst the increase in $f/n$ has adversarial effects on the fault-tolerance, the increase in the batch-size improves the fault-tolerance for any given fraction of faults. At large, the observed effects on the fault-tolerance achieved by the CGE gradient-filter to change in the fraction of faults $f/n$ is coherent with the theoretical analysis presented in Section~\ref{sec:ft}.\\



% \subsubsection{CIFAR-10 Dataset}
% \label{subsub:cifar}

{\bf CIFAR-10:} We present below experimental results for CIFAR-10 which is also an image-classification dataset that comprises $60,000$ color images belonging $10$ mutually exclusive categories~\cite{krizhevsky2009learning}. The dataset is further divided into $50,000$ training samples and $10,000$ testing samples. Learning on CIFAR-10 is more challenging than on MNIST, since the images in MNIST are monochromatic and has less variety, while the images in CIFAR-10 are quite diverse. 
% For instance, images of different breeds of dogs can look very differently from each other. 
Similar to MNIST, we consider the convolutional neural network $\mathsf{LeNet}$ with $657,080$ learning parameters. Thus, the value of dimension $d = 657,080$ in this case. We consider $n = 40$ agents in the system. Our experimental results for the different gradient-filters in the presence of $f= 8$ faulty agents exhibiting different types of faults are shown in Figure~\ref{fig:cifar-fault-type-01}. \\

\begin{figure}[tb!]
    \centering
    \includegraphics[width=\linewidth]{Experiments/aaai/cifar/cifar-comparison-5.pdf}
    %\includegraphics[width=\linewidth]{Experiments/aaai/cifar/cifar-comparison-2.pdf}
    \caption{\footnotesize{\it Distributed learning of $\mathsf{LeNet}$ for CIFAR-10 dataset using the D-SGD method with batch size $k=64$ and the different gradient-filters (represented using different colors) in the presence of $f = 8$ faulty agents exhibiting different Byzantine faults.}}
    \label{fig:cifar-fault-type-01}
\end{figure}

\begin{figure}[tb!]
    \centering
    \includegraphics[width=\linewidth]{Experiments/aaai/averaging/averaging-comparison-5.pdf}
    %\caption{\footnotesize{\it Performance comparison of CGE filter for distributed learning of neural networks for MNIST dataset using gradient averaging D-SGD method with batch size $k=64$ in presence of faulty agents exhibiting \emph{norm-confusion} type of Byzantine faults. \emph{no ave.} indicates the case where gradient averaging is not used. Values calculated by averaging the 475th to 500th steps in each experiment.}}
    \caption{\footnotesize{\it Average training losses and testing accuracies evaluated between $475$ to $500$ steps of the D-SGD method with CGE gradient-filter for distributed learning of the neural network $\mathsf{LeNet}$ (for the MNIST dataset) in the presence of different number of faulty agents $f$ (represented by different colors) when applying \emph{exponential averaging} of stochastic gradients for different values of $\alpha$. \emph{no ave.} indicates the case when no averaging is not used. Here, the data batch-size $k = 64$, and the fault type is \emph{norm-confusing}.}}
    \label{fig:averaging-01}
\end{figure}

\begin{figure}[tb!]
    \centering
    \includegraphics[width=\linewidth]{Experiments/aaai/averaging/averaging-detail-1.pdf}
    \caption{\footnotesize{\it Distributed learning of $\mathsf{LeNet}$ for MNIST dataset using the D-SGD method with batch size $k=64$ and CGE gradient-filter in the presence of $f = 8$ and $10$ faulty agents exhibiting \emph{norm-confusing} type of faults. \emph{Exponential averaging} of stochastic gradients applied with different values of $\alpha$  (represented using different colors).}}
    \label{fig:averaging-detail}
\end{figure}

% mentio~\ref{fig:batch-size-3} and Figure~\ref{fig:batch-size-4}, we note that multi-KRUM works generally handles \textit{reverse} and \textit{norm-confusing} with a similar capability, while it becomes more difficult when number of faulty agents is larger under \textit{norm-confusing}. There is a significant improvement under both fault types when batch size increases from 16 to 64. With batch size being 64, it is with higher probability that good agents, drawn with identical independent distribution, would return a group of gradients with lower variance in a step. This also confirms our proposition in the previous subsection, that multi-KRUM works better when the variance of good gradients are lower.\\

% Similarly, comparing Figure~\ref{fig:batch-size-4} and Figure~\ref{fig:batch-size-5}, we see that CGE handles \textit{reverse} better than \textit{norm-confusing}, which is understandable since \textit{reverse} provides faults that are more distinguishable to CGE. Meanwhile, we don't see a similar instability of multi-KRUM when facing more faulty agents under \textit{norm-confusing}, that batch size does not effect performance of CGE significantly. \\





% When fraction of faulty agents is larger or equal to 50\%, the fault-tolerant task become meaningless. For comparison purpose, we also document a group of results for reference, where no gradient filter is applied, that only plain averaging is used upon receiving gradients from agents, in Appendix \ref{sub:exp-with-no-filter}. \\

% It is shown in the Figures that CGE is generally more stable than multi-KRUM, that in most cases, SGD would converge rapidly and to a value that is close to the fault-free convergence, while multi-KRUM might take more steps, and there might be a gap between the value SGD converges to and the value of fault-free convergence. Notice that when batch size increases such gap is become smaller, but as is shown by plots in Figure~\ref{fig:fault-fraction-4}, the gap still exists when batch size is larger.\\

% One thing worth noticing, which is also observed in previous experiments, is that SGD under both filters shows the unstable behavior we have seen previously, under \textit{coordinate-wise} type of fault, regardless of batch size, but only when the number of faulty agents is 1 or 2. When the fraction of faulty agents become larger, the training loss become stable instead. Notice that under \textit{coordinate-wise} fault, faulty agents produce their bad gradients collaboratively but everyone of them produces the same bad gradient in each step; which might be the reason since the bad gradients become easier for filters to spot when there are more of them.

\iffalse
\begin{figure*}[p]
    \centering
    \includegraphics[width=\textwidth]{Experiments/new/fault_fraction_comparison/num-faults-comparison-1.pdf}
    \caption{ Distributed learning of neural networks for MNIST dataset using the D-SGD method and the CGE gradient-filter under different number of faulty agents $f$ out of $n = 10$. In these experiments the data batch-size $k = 16$. Different rows present different fault types: (a) \textit{gadient reverse}, (b) \textit{coordinate-wise}, (c) \textit{norm-confusing}, (d) \textit{label-flipping}, and (e) \textit{random}. The two columns plot the training loss and the testing accuracy, respectively.}
    \label{fig:fault-fraction-1}
\end{figure*}
\begin{figure*}[p]
    \centering
    \includegraphics[width=\textwidth]{Experiments/new/fault_fraction_comparison/num-faults-comparison-2.pdf}
    \caption{Distributed learning of neural networks for MNIST dataset using the D-SGD method and the multi-KRUM ($m=2$) gradient-filter under different number of faulty agents $f$ out of $n = 10$. In these experiments the data batch-size $k = 16$. Different rows present different fault types: (a) \textit{gadient reverse}, (b) \textit{coordinate-wise}, (c) \textit{norm-confusing}, (d) \textit{label-flipping}, and (e) \textit{random}. The two columns plot the training loss and the testing accuracy, respectively.}
    \label{fig:fault-fraction-2}
\end{figure*}
\begin{figure*}[p]
    \centering
    \includegraphics[width=\textwidth]{Experiments/new/fault_fraction_comparison/num-faults-comparison-3.pdf}
    \caption{Distributed learning of neural networks for MNIST dataset using the D-SGD method and the CGE gradient-filter under different number of faulty agents $f$ out of $n = 10$. In these experiments the data batch-size $k = 64$. Different rows present different fault types: (a) \textit{gadient reverse}, (b) \textit{coordinate-wise}, (c) \textit{norm-confusing}, (d) \textit{label-flipping}, and (e) \textit{random}. The two columns plot the training loss and the testing accuracy, respectively.}
    \label{fig:fault-fraction-3}
\end{figure*}
\begin{figure*}[p]
    \centering
    \includegraphics[width=\textwidth]{Experiments/new/fault_fraction_comparison/num-faults-comparison-4.pdf}
    \caption{Distributed learning of neural networks for MNIST dataset using the D-SGD method and the multi-KRUM ($m=2$) gradient-filter under different number of faulty agents $f$ out of $n = 10$. In these experiments the data batch-size $k = 64$. Different rows present different fault types: (a) \textit{gadient reverse}, (b) \textit{coordinate-wise}, (c) \textit{norm-confusing}, (d) \textit{label-flipping}, and (e) \textit{random}. The two columns plot the training loss and the testing accuracy, respectively.}
    \label{fig:fault-fraction-4}
\end{figure*}
\fi

%\newpage

Finally, we present below an {\em exponentially weighted averaging} scheme for stochastic gradients that aims to improve the fault-tolerance achieved by a gradient-filter.

% We use the same class of convolutional neural networks $\mathsf{LeNet}$, as for the MNIST dataset above, and perform similar experiments. 

% Some of the results are documented here in Figure~\ref{fig:cifar-1}. As CIFAR-10 is a more difficult task to MNIST and we are using the same neural network, we see that the speed of convergence is much slower than what we have in MNIST, and with the same 300 steps, we can only see a trend of convergence. But still, some filters works better than others. Geometric median (a), median of means (b), and coordinate-wise trimmed mean (c) cannot handle the case where there are 4 out of 10 fault agents. There is a gap between multi-KRUM plots and fault-free plot, while CGE, out of the five filters, help SGD converge with a speed close to the fault-free case. The relative performance of filters are basically the same as in MNIST, that CGE works generally better than mutli-KRUM no matter which dataset is using.\\

\iffalse
\begin{figure*}[p]
    \centering
    \includegraphics[width=\textwidth]{Experiments/new/cifar_comparison/cifar-filter-comparison-1.pdf}
    \caption{Distributed learning of neural networks for CIFAR-10 dataset using the D-SGD method and the different gradient-filters in presence of $f = 1$ faulty agent, out of $n=10$ total agents, exhibiting the \textit{coordinate-wise} faults. In these experiments the data batch-size $k = 16$. Different rows correspond to different gradient-filters: (a) geometric median, (b) median of means, (c) coordinate-wise trimmed mean, (d) multi-KRUM with $m=2$, and (e) CGE.}
    \label{fig:cifar-1}
\end{figure*}
\fi

\subsection{Exponential averaging of stochastic gradients}
\label{sub:appendix_averaging}

We observe from our experiments above, specifically the plots in Figure~\ref{fig:batch-size-01}, that fault-tolerance of CGE gradient-filter improves with increase in the data batch-size $k$. The reason why this happens is the fact that larger batch-size results in stochastic gradients with smaller variances $\sigma^2$, which, owing to our results in Section~\ref{sec:ft}, results in improved fault-tolerance. However, increase in data batch-size also increases the cost of computing stochastic gradients in each iteration. Motivated from this observation, we propose a more economical technique of {\em exponential averaging} that allows the non-faulty agents to compute stochastic gradients with reduced variances without increasing data batch-size and their cost for computing the stochastic gradients. Alternately, we may also use other existing variance reduction techniques from the stochastic optimization literature~\cite{bottou2018optimization}.\\

% Similar theoretical observations have also been made for the other gradient-filters~\cite{blanchard2017machine, chen2017distributed, yin2018byzantine}. 
% In general, fault-tolerance of a gradient-filter improves with decreasing variances of the non-faulty stochastic gradients.\\
% by using gradient-filters is quite sensitive to the individual agents' data batch-sizes. In the case of distributed learning with CGE gradient-filter, the training loss in presence of faults improves significantly when batch-size increases. 


For each iteration $t$ and agent $i$, the server maintains an {\bf exponentially weighted average} $h^t_i$ of the stochastic gradients received from agent $i$ so far. Specifically, for $\alpha \in [0, \, 1)$,
\begin{align}
    h^t_i = \alpha\, h^{t-1}_i + (1-\alpha) \, g^t_i. \label{eqn:grad_avg_scheme}
\end{align}
where $g^t_i$ denotes the stochastic gradient received by the server from agent $i$ in iteration $t$. Given a set of $n$ vectors $y_1, \ldots, \, y_n$, let $\mathsf{CGE}_f\{y_1, \ldots, \, y_n\}$ denote the output of our CGE gradient-filter defined in step {S2} of Algorithm~\ref{alg:cge}. 
% , i.e.,
% \[\mathsf{CGE}_f\{y_1, \ldots, \, y_n\} = \sum_{j = 1}^{n-f} y_j.\]
For each iteration $t$, in step {S2} of Algorithm~\ref{alg:cge} the server updates the current estimate $w^t$ to
\[w^{t+1} = w^{t} + \eta_t\cdot\mathsf{CGE}_f\left\{h^t_1, \ldots, \, h^t_n \right\}.\]
% Recall that $\eta_t$ is the step-size for iteration $t$. 
It should be noted that the above averaging scheme does not increase the per iteration computation cost for an individual agent, unlike the case when we increase the data batch-size.\\

% for reducing the variance of stochastic gradients. \\
% When $\alpha = 0$ then the above gradient averaging scheme reduces to the conventional stochastic gradient method.

% then positive   
% the experimental results for the gradient c which impro
% Another way of address this problem might be using a gradient averaging scheme. By averaging previous steps gradients collected from each agent, it is expected to reduce variance among good agents, so that gradients from fault agents become more distinguishing to filters. Let $h^t_j$ denote the averaging history of gradients of agent $t$ at step $j$, $0\leq\alpha\leq1$,
% $$h^t_j = \alpha\cdot h^{t-1}_j + (1-\alpha) g^t_j$$
% Update parameters by the following scheme instead of:
% $$w^t = w^{t-1} + \mu\cdot\mathrm{Filter}_j\{h^t_j\}$$
% Note that under this definition, $\alpha=0$ indicates plain SGD with no averaging.

To evaluate the impact of the above exponential averaging on the fault-tolerance of CGE gradient-filter, we introduce a new type of fault designed deliberately against our CGE filter:

\noindent \textbf{Norm-confusing fault}: Similar to gradient-reverse fault, a faulty agent sends to the server a vector directed opposite to its correct stochastic gradient. However, in this particular type of fault, the norm of the vector is scaled to the $(f+1)$-th largest norm amongst the stochastic gradients of all the $n-f$ non-faulty agents. 

Experiments are conducted on the distributed learning of $\mathsf{LeNet}$ neural networks for MNIST dataset with $k = 64$ and different values of $f$. The outcomes are shown in Figures~\ref{fig:averaging-01}. Smaller training loss can be achieved with exponential averaging and larger value of $\alpha$ in the same number of steps. Figure~\ref{fig:averaging-detail} further shows that even if there are larger number $f$ of faulty agents in the system and plain CGE converges slowly, exponential averaging can still significantly improve the performance. As shown in Table~\ref{tab:ave-run-time}, exponential averaging does not have a significant impact on the running time.\\
%In particular, upon comparing Figures~\ref{fig:batch-size-01} and~\ref{fig:averaging-01}, we note that the fault-tolerance with data batch-size $k = 64$ with temporal averaging is comparable to fault-tolerance with data batch-size $k = 256$ without temporal averaging. 

Experiments also show that exponential averaging improves the fault-tolerance performance of other gradient-filters. For example, Figure~\ref{fig:averaging-detail-cwtm} shows the outcome of distributed learning of \textsf{LeNet} neural networks for MNIST dataset with $k=64$ and $f=10$, using median-of-means and coordinate-wise trimmed mean filters. With exponential averaging and larger value of $\alpha$, faster convergence can be achieved for both filters.

\begin{table}[tb!]
    \centering
    \caption{\footnotesize{Running time for distributed learning of \textsf{LeNet} for MNIST using D-SGD method with batch size $k=64$ and the different gradient-filters in presence of $f=8$ faulty agents exhibiting \emph{norm-confusing} type of fault with or without applying \emph{exponential averaging} for different values of $\alpha$, corresponding to the training process shown in Fig.~\ref{fig:averaging-detail}(a). Total running time refers to the time for 500 iterations.}}
    \footnotesize
    \begin{tabular}{c|cc}
        \textbf{Filter} & \textbf{Time per iteration} (s) & \textbf{Total running time} (s) \\
        \hline
        CGE (No ave.) & 0.613 & 306.9 \\
        CGE ($\alpha=0.2$) & 0.733 & 366.7 \\
        CGE ($\alpha=0.4$) & 0.731 & 365.5 \\
        CGE ($\alpha=0.6$) & 0.733 & 366.7 \\
    \end{tabular}
\label{tab:ave-run-time}
\end{table}

\begin{figure}[tb!]
    \centering
    \includegraphics[width=\linewidth]{Experiments/aaai/averaging/averaging-detail-3.pdf}
    \caption{\footnotesize{\it Distributed learning of $\mathsf{LeNet}$ for MNIST dataset using the D-SGD method with batch size $k=64$ and different gradient-filters in the presence of $f = 10$ faulty agents exhibiting \emph{norm-confusing} type of faults. \emph{Exponential  averaging} of stochastic gradients applied with different values of $\alpha$  (represented using different colors). Filters used here are \emph{(a)} median-of-means (\emph{MoM}), and \emph{(b)} coordinate-wise trimmed mean (\emph{CWTM}).}}
    \label{fig:averaging-detail-cwtm}
\end{figure}

% omparing to when gradient averaging is not used (\textit{no ave.}, the same as markers for $k=64$ in Figure~\ref{fig:batch-size-01}), the final loss of the training process improves with gradient averaging. Moreover, we also observe that the fault-tolerance achieved by CGE  gradient-filter further improves with increase in the value of $\alpha$. 

% The value of $\alpha$ varies between 0 and 0.60. Comparing plots in each figure, it is easy to find that with an increase of the value of $\alpha$, the pike in loss (or dive in accuracy) become less significant and less frequent. Also, convergence speed does not change much with increasing of $\alpha$. In Figure~\ref{fig:accumulation-1}(b), we see that this averaging scheme can sometimes also helps SGD avoid a worse local minimum.

% Similarly to what we do in Section \ref{sub:appendix_averaging}, we can also apply averaging scheme on CIFAR-10 tasks, where due to the variety of training samples, the variance of gradients would be even higher than in MNIST. Figures~\ref{fig:cifar-accumulation-1} and \ref{fig:cifar-accumulation-2} presents the results. Comparing to plots in Figure~\ref{fig:cifar-1}(d) and \ref{fig:cifar-1}(e), we see that the turbulence also reduces when value of $\alpha$ increases, regardless of the filter. We also notice that there is a small gap between plots of multi-KRUM and the fault-free plot, while averaging would further help CGE eliminate that gap.


==> experiments_averaging.tex <==
\subsection{Gradient averaging}
\label{sub:appendix_averaging}

We observe from the experiments above, specifically the plots in Figures~\ref{fig:batch-size-3},~\ref{fig:batch-size-4},~\ref{fig:batch-size-5} and~\ref{fig:batch-size-6}, that fault-tolerance by using gradient-filters is quite sensitive to the individual agents' data batch-sizes. For instance, consider the case of distributed learning with CGE gradient-filter in presence of faulty agents exhibiting \textit{coordinate-wise} faults shown in Figure~\ref{fig:fault-fraction-1}(b). Although the different between the training losses in presence and in absence of faults is small for more iterations (or steps), the training loss in presence of faults is littered with spikes even in the later stages of the learning process. However, we observe that the magnitude of these spikes attenuates significantly when we increase the data batch-size $k$ from $16$ to $64$, as shown in Figure~\ref{fig:fault-fraction-3}(b). The reason why this happens is the fact that larger is the batch-size for computing the stochastic gradients smaller is the variance $\sigma^2$, and therefore, as per our theoretical analysis presented in Section~\ref{sub:ft}, better is the fault-tolerance by the CGE gradient-filter. Similar theoretical observations have also been made for the other gradient-filters~\cite{blanchard2017machine, chen2017distributed, yin2018byzantine}. In general, it is safe to say that fault-tolerance of a gradient-filter improves if the variance $\sigma^2$ of the stochastic gradients computed by the non-faulty agents reduces.\\

% We noticed that in previous experimental results, there are `unstable' behaviors shown in the plots, especially when under the fault type of \textit{coordinate-wise}. We can see that in some cases, for example, $f=0$ or $1$ in Figure~\ref{fig:fault-fraction-1}(b), t

Motivated from the above observations, we propose a technique of {\em gradient averaging} below that allows the non-faulty agents to compute stochastic gradients with reduced variance $\sigma^2$ without increasing their data batch-size $k$. Now, it should be noted that for reducing the variance of the stochastic gradients we could also use other existing variance reduction techniques from the stochastic optimization literature~\cite{bottou2018optimization}. For now, we consider the gradient averaging presented below.\\

For each iteration $t$ and agent $i$, let $h^t_i$ denote the weighted average of the stochastic gradients received till the $t$-th iteration by the server from agent $i$. Specifically, let $\alpha \in [0, \, 1)$ and let $g^t_i$ denote the stochastic gradient received from agent $i$ in iteration $t$. Then, for each agent $i$ and iteration $t$,
\begin{align}
    h^t_i = \alpha\, h^{t-1}_i + (1-\alpha) \, g^t_i. \label{eqn:grad_avg_scheme}
\end{align}
Given a set of $n$ vectors $y_1, \ldots, \, y_n$, let $\mathsf{Filter}\{y_1, \ldots, \, y_n\}$ denote the output of a gradient-filter, such as CGE or multi-KRUM. Then, in step {\bf S2} of each iteration $t$ of the D-SGD algorithm presented in Section~\ref{sub:steps}, the server updates the current estimate $w^t$ to 
\[w^t = w^{t-1} + \eta_t\cdot\mathsf{Filter}\left\{h^t_1, \ldots, \, h^t_n \right\}.\]
Recall that $\eta_t$ is the step-size for iteration $t$. It should be noted that the above averaging scheme does not increase the per iteration computation cost for an individual agent, unlike the case when we increase the data batch-size for reducing the variance of stochastic gradients. \\
% When $\alpha = 0$ then the above gradient averaging scheme reduces to the conventional stochastic gradient method.

% then positive   
% the experimental results for the gradient c which impro
% Another way of address this problem might be using a gradient averaging scheme. By averaging previous steps gradients collected from each agent, it is expected to reduce variance among good agents, so that gradients from fault agents become more distinguishing to filters. Let $h^t_j$ denote the averaging history of gradients of agent $t$ at step $j$, $0\leq\alpha\leq1$,
% $$h^t_j = \alpha\cdot h^{t-1}_j + (1-\alpha) g^t_j$$
% Update parameters by the following scheme instead of:
% $$w^t = w^{t-1} + \mu\cdot\mathrm{Filter}_j\{h^t_j\}$$
% Note that under this definition, $\alpha=0$ indicates plain SGD with no averaging.

To evaluate the impact of gradient averaging on fault-tolerance by gradient-filter, we repeat the above experiments on the distributed learning of $\mathsf{LeNet}$ neural networks for MNIST and CIFAR-10 datasets. The outcomes of some of our experiments are shown below in Figures~\ref{fig:accumulation-1},~\ref{fig:accumulation-2},~\ref{fig:cifar-accumulation-1} and \ref{fig:cifar-accumulation-2}. We observe that in general the stability of the learning process improves with gradient averaging, and especially for the case when the faulty agents exhibit the {\em coordinate-wise} faults, as shown in Figures~\ref{fig:accumulation-1}(b),~\ref{fig:accumulation-2}(b),~\ref{fig:cifar-accumulation-1}(b) and~\ref{fig:cifar-accumulation-2}(b). Moreover, we also observe that the fault-tolerance achieved by a gradient-filter improves with increase in the value of $\alpha$. 

% The value of $\alpha$ varies between 0 and 0.60. Comparing plots in each figure, it is easy to find that with an increase of the value of $\alpha$, the pike in loss (or dive in precision) become less significant and less frequent. Also, convergence speed does not change much with increasing of $\alpha$. In Figure~\ref{fig:accumulation-1}(b), we see that this averaging scheme can sometimes also helps SGD avoid a worse local minimum.

% Similarly to what we do in Section \ref{sub:appendix_averaging}, we can also apply averaging scheme on CIFAR-10 tasks, where due to the variety of training samples, the variance of gradients would be even higher than in MNIST. Figures~\ref{fig:cifar-accumulation-1} and \ref{fig:cifar-accumulation-2} presents the results. Comparing to plots in Figure~\ref{fig:cifar-1}(d) and \ref{fig:cifar-1}(e), we see that the turbulence also reduces when value of $\alpha$ increases, regardless of the filter. We also notice that there is a small gap between plots of multi-KRUM and the fault-free plot, while averaging would further help CGE eliminate that gap.



\begin{figure}[p]
    \centering
    \includegraphics[width=\textwidth]{Experiments/new/accumulation_comparison/averaging-comparison-1.pdf}
    \caption{Distributed learning of neural networks for MNIST dataset using the D-SGD method with gradient averaging and the multi-KRUM ($m=2$) gradient-filter in presence of Byzantine faulty agents exhibiting the \textit{coordinate-wise} faults. The different values of weight $\alpha$ are mentioned at the top. For all these experiments we used data batch-size $k = 16$. Different rows correspond to different number of faults: (a) $f=1$, (b) $f=2$, (c) $f=3$, and (d) $f=4$.}
    \label{fig:accumulation-1}
\end{figure}

\begin{figure}[p]
    \centering
    \includegraphics[width=\textwidth]{Experiments/new/accumulation_comparison/averaging-comparison-2.pdf}
    \caption{Distributed learning of neural networks for MNIST dataset using the D-SGD method with gradient averaging and the CGE gradient-filter in presence of Byzantine faulty agents exhibiting the \textit{coordinate-wise} faults. The different values of weight $\alpha$ are mentioned at the top. For all these experiments we used data batch-size $k = 16$. Different rows correspond to different number of faults: (a) $f=1$, (b) $f=2$, (c) $f=3$, and (d) $f=4$.}
    \label{fig:accumulation-2}
\end{figure}

\begin{figure}[p]
    \centering
    \includegraphics[width=\textwidth]{Experiments/new/cifar_comparison/cifar-averaging-comparison-1.pdf}
    \caption{Distributed learning of neural networks for CIFAR-10 dataset using the D-SGD method with gradient averaging and the multi-KRUM ($m=2$) gradient-filter in presence of Byzantine faulty agents exhibiting the \textit{coordinate-wise} faults. The different values of weight $\alpha$ are mentioned at the top. For all these experiments we used data batch-size $k = 16$. Different rows correspond to different number of faults: (a) $f=1$, (b) $f=2$, (c) $f=3$, and (d) $f=4$.}
    \label{fig:cifar-accumulation-1}
\end{figure}

\begin{figure}[p]
    \centering
    \includegraphics[width=\textwidth]{Experiments/new/cifar_comparison/cifar-averaging-comparison-2.pdf}
    \caption{Distributed learning of neural networks for CIFAR-10 dataset using the D-SGD method with gradient averaging and the CGE gradient-filter in presence of Byzantine faulty agents exhibiting the \textit{coordinate-wise} faults. The different values of weight $\alpha$ are mentioned at the top. For all these experiments we used data batch-size $k = 16$. Different rows correspond to different number of faults: (a) $f=1$, (b) $f=2$, (c) $f=3$, and (d) $f=4$.}
    \label{fig:cifar-accumulation-2}
\end{figure}

==> prior.tex <==
\section{Related Work}
\label{sec:prior}
In this subsection, we present comparisons between our contributions and that of the related prior works on fault-tolerance in distributed machine learning.\\

The idea of norm-based gradient filtering was originally proposed for conferring fault-tolerance to the distributed {\em gradient-descent} method when solving the multi-agent {\em distributed optimization} problem~\cite{gupta2019byzantine}. However, unlike the distributed gradient-descent method, in the D-SGD method the agents can only compute {\em stochastic gradients} which are noisy estimates of the actual gradients of their individual loss functions. 
% Therefore, the fault-tolerance property of the CGC filter when applied to the D-SGD method is not obvious from the results presented in the technical report~\cite{bottou2018optimization}. 
A detailed description of the resulting D-SGD algorithm with the CGE gradient filter, and its formal fault-tolerance properties are presented in Section~\ref{sec:algo}. The algorithm schematic is shown in Figure~\ref{fig:algo}. \\

Subsequent to the initial work on fault-tolerance in distributed {\em optimization} by Su and Vaidya~\cite{su2016fault}, the problem of fault-tolerance in distributed {\em learning} has gained significant attention in recent years~\cite{alistarh2018byzantine, bernstein2018signsgd, blanchard2017machine, cao2019distributed, chen2017distributed, damaskinos2018asynchronous, data2020byzantine, rajput2019detox, xie2018generalized, xie2019zeno, yang2017byrdie}. The distributed learning problem can be modeled as a special case of the more general distributed optimization problem where the cost function (or the loss function) for each non-faulty agent is equal to the expected loss function defined in~\eqref{eqn:exp_loss}. However, unlike distributed optimization, in distributed learning the agents may only compute {\em approximate or noisy} gradients of their individual expected loss functions. Therefore, it is non-trivial to extend the applicability of the algorithms originally proposed for fault-tolerance in distributed optimization, such as the ones in~\cite{gupta2019byzantine, gupta2020resilience, su2016fault, sundaram2018distributed}, to fault-tolerance in distributed machine learning. \\

 It should be noted that exact fault-tolerance in distributed optimization is achievable in presence of up to $f$ faulty agents if and only if the non-faulty agents' cost functions satisfy the {\em $2f$-redundancy} property~\cite{gupta2020fault_podc, gupta2020resilience}. In the case of homogeneous distributed learning problem, described above in Section~\ref{sec:intro}, as the non-faulty agents' expected loss functions are identical, the {\em $2f$-redundancy} property is naturally satisfied if $n > 2f$. Therefore, in principle, we can compute an optimal learning parameter defined by~\eqref{eqn:obj} despite the presence of some Byzantine faulty agents as long as the faulty agents are in the minority. However, note that in pragmatic distributed learning settings, the agents may only be able to compute and send to the server partial information about their individual expected loss functions. In most cases, the partial information is in the form of {\em stochastic gradients}. Therefore, even if exact fault-tolerance is feasible in theory, its achievability relies on additional assumptions besides {\em $2f$-redundancy} as is evident from prior work on this problem~\cite{bernstein2018signsgd, blanchard2017machine, data2020byzantine, gupta2019byzantine_sgd, xie2019zeno}.\\

The CGE gradient-filter studied in this report was originally proposed and studied for fault-tolerance in the generic distributed {\em optimization} setting in our prior work~\cite{gupta2019byzantine, gupta2020fault_podc}. In the problem of distributed optimization, different agents have different cost functions. Alternately, the setting of distributed optimization considered in~\cite{gupta2019byzantine, gupta2020fault_podc} is equivalent to the setting of {\em heterogeneous} distributed learning wherein different agents could sample data points from different probability distributions, unlike in the setting of homogeneous learning described above in Section~\ref{sec:intro}. However, in our prior work we assume that the agents compute {\em true} gradients of their individual cost functions to the server. In the learning setting the agents can only compute {\em stochastic} gradients, i.e., noisy estimates of the true gradients. An extended applicability of the CGE gradient-filter to fault-tolerance in stochastic gradient-descent based distributed {\em linear regression} was presented in~\cite{gupta2019byzantine_sgd}. In the current report, however, we consider a more general learning setting than linear regression wherein the expected loss function $Q(w)$ is an arbitrary strongly convex function with Lipschitz continuous gradients. Moreover, through experiments in the current report we have also demonstrated the applicability of the CGE gradient-filter to fault-tolerance in distributed learning of artificial neural networks wherein the function $Q(w)$ may be non-convex. \\

In recent years, several other gradient-filters have been proposed and studied for fault-tolerance in the D-SGD method based distributed learning. For all these gradient-filters, including the CGE gradient-filter, in each iteration the server replaces the aggregate of the received stochastic gradients in~\eqref{eqn:update} with a {\em robust estimate} of the aggregate of the non-faulty stochastic gradients. For instance, in the multi-KRUM gradient-filter the server uses the aggregate of only a few stochastic gradients (out of the $n$) received depending upon their proximity to each other~\cite{blanchard2017machine}. In the geometric median of means gradient-filter~\cite{chen2017distributed}, and the SVD based gradient-filter~\cite{data2020byzantine, diakonikolas2018sever, prasad2018robust}, the server implements standard agnostic mean estimation techniques from the robust statistics literature~\cite{charikar2017learning, huber2011robust}. The coordinate-wise trimmed mean gradient-filter~\cite{yang2017byrdie, yin2018byzantine} is an extension of the truncated mean filter which was originally proposed for scalar gradients~\cite{su2016fault} to the case of higher-dimensional stochastic gradients.\\

Gradient filtering based on their Euclidean norms (or magnitude), similar to the CGE gradient-filter, has been studied recently for fault-tolerance in the distributed learning problem~\cite{ghosh2019communication}. In~\cite{ghosh2019communication}, however, each agent samples apriori a finite number of data points from the probability distribution $\D$, and then sends to the server in each iteration the {\em true} gradient, instead of a {\em stochastic} gradient, of its individual expected loss function. Ghosh et al.~\cite{ghosh2019communication} has shown that norm-based gradient filtering achieves order optimal {\em statistical error rate}, in presence of Byzantine faulty agents, if the probability distribution of data points $\D$ is Gaussian and the true gradients of the agents' individual expected loss functions have a {\em sub-exponential} probability distribution. In the current report, we consider a more pragmatic setting wherein the non-faulty agents may only send independently computed {\em stochastic} gradients of the expected loss function $Q(w)$ to the server, and we do not make any assumptions about the probability distribution $\D$ of data points.\\

% Importantly, the computational complexity of our proposed fault-tolerance mechanism, i.e., the CGC gradient-filter, is $\mathcal{O}(n (d + \log n))$, which is significantly lower than that of the fault-tolerance mechanisms proposed in some of these prior works~\cite{alistarh2018byzantine, blanchard2017machine, chen2017distributed, cao2019distributed}. Moreover, our algorithm applies to more general distributed learning settings that satisfy $2f$-redundancy.\\
 % We can tolerate a high fraction of faulty agents when the condition number is small, and vice-versa. \\


% Besides the fact that we consider the more general setting of distributed optimization, in the context of distributed sensing we only assume the $2f$-redundancy property for deriving the fault-tolerance guarantee of our algorithm.\\

Finally, we also note that norm-based gradient elimination similar to the CGE gradient-filter has been utilized in the past for solving unrelated problems, such as mitigating the impact of {\em gradient explosion} and controlling the privacy-accuracy trade-offs in {\em differential privacy} protocols, in the D-SGD method~\cite{pascanu2012understanding, shokri2015privacy}. We use norm-based gradient elimination for Byzantine fault-tolerance. Besides this difference in the objectives, unlike these past works, we use a {\em dynamic} (or adaptive) threshold for eliminating the gradients instead of a {\em static} threshold. This difference is critical for the fault-tolerance property of the CGE gradient-filter.


%\footnote{In the centralized setting of this problem, the responses are often formulated as $Y = X w^* + B$, where $(X,\, Y)$ represents the data points and responses, and $B$ represents a sparse adversarial (Byzantine) corruption-vector~\cite{bhatia2015robust}.}
%It should be noted that Byzantine fault tolerance is not the same as robustness to arbitrary outliers as modeled in~\cite{prasad2018robust,diakonikolas2018sever}, mainly because Byzantine faulty agents can (actively) adapt to robustness techniques, run by the server, and mislead the server to a parameter value of their choice~\cite{bhatia2015robust, blanchard2017machine}. 
%In fact, the server could be completely unaware of the data points held by any agent in the system. 

% \subsubsection{Challenges of distributed over centralized setting}
% The challenges of distributed setting over the centralized counterpart are as follows.
% \begin{enumerate}
% \item Both the data points and responses of Byzantine faulty agents can be corrupted. Some of the centralized techniques (cf. \cite{bhatia2015robust, mcwilliams2014fast}) assume only corrupted responses. 

% \item Agents could be holding large volume of data points and responses, that would make sharing of the entire data set with the server quite expensive in terms of the communication cost. Most of the centralized techniques (cf.~\cite{bhatia2015robust}) require the server to have access to all the agents' data points and responses. 

%\item Corruptions in the data points and responses of the server need not be static, i.e. Byzantine faulty agents can corrupt their data points (or responses) dynamically during the execution of a regression algorithm~\cite{su2018finite, blanchard2017machine}. None of the centralized techniques consider dynamic corruptions.

% \item Server and the agents need not be synchronous. All the centralized techniques rely on synchronicity in the system~\cite{bhatia2015robust, chen2013robust, mcwilliams2014fast, prasad2018robust, diakonikolas2018sever}. 
% \end{enumerate}

% Unlike the centralized techniques, our proposed algorithms do not require agents to share their data points or responses with the server, and it is \emph{partially asynchronous}.
% %Thus, in our problem setting, nothing can be assumed about the data points or responses of Byzantine-faulty agents.  
% While spectral filters proposed in~\cite{prasad2018robust, diakonikolas2018sever} can be used in the distributed setting, they rely on singular value decomposition (SVD) of agents' costs' gradients (in each iteration) and therefore, are orders of magnitude more computationally complex than the proposed norm based filters. Also, unlike~\cite{prasad2018robust, diakonikolas2018sever}, we are interested in computing $w^*$ precisely (in absence of noise and within a reasonably bounded error in presence of noise) in a deterministic manner. \\

% The `hard-thresholding' based robust regression technique in~\cite{bhatia2015robust}, even for the centralized setting, is effective only if the data points satisfy a certain condition. This condition holds with ``high probability" if the probability distribution of the data points is Gaussian with zero mean~\cite{bhatia2015robust}. It should be noted that the efficacy of our proposed algorithms does not depend on any assumptions on the probability distribution of agents' data points. Therefore, the proposed algorithms have a much wider applicability than the solutions proposed in~\cite{bhatia2015robust}, even for the centralized case.

% \subsection{Byzantine fault tolerant distributed estimation}
% In a closely related work, Su and Shahrampour~\cite{su2018finite} propose \emph{coordinate-wise trimmed mean} filtering for ``robustifying" the distributed gradient descent method in a peer-to-peer network. However, they do not provide an explicit bound on the number of Byzantine faulty agents that can be tolerated using their filtering technique. The convergence of their algorithm relies on a technical assumption (assumption 1 in~\cite{su2018finite}) that imposes additional constraints, than required by our proposed algorithms, on agents' data points. This point is reiterated by an example in Section~\ref{sec:num}. Resilient estimation technique proposed by~\cite{chen2018resilient} requires agents to commit (or share) their data points and responses to the server (or some central authority in their case), whereas we are interested in distributed setting where agents do not share their data points or responses with the server or any other agent in the system. In recent years, there has been a significant amount of work in Byzantine fault-tolerant state estimation (both distributed and centralized) of linear time-invariant (LTI) dynamical systems~\cite{mitra2018byzantineresilient,fawzi2014secure, shoukry2017secure,pajic2017attack, ren2019secure}. However, it should be noted that Byzantine fault-tolerant state estimation (aka. secure state estimation) of LTI dynamical systems is a special case of the considered regression problem (ref.~\cite{mitra2018byzantineresilient,fawzi2014secure, shoukry2017secure,pajic2017attack, ren2019secure}). We also note that our proposed algorithms are significantly (orders of magnitude) simpler than some of the secure state estimation algorithms~\cite{shoukry2017secure,pajic2017attack}, albeit can handle relatively less number of Byzantine faulty agents.

%Authors in~\cite{mitra2018byzantineresilient} address the problem of Byzantine fault tolerant  \emph{observer}, in peer-to-peer network setting, for linear time-invariant (LTI) dynamical systems, and so in general, their technique is not applicable to the considered distributed regression problem.

% \def\krum{{\sf Krum}}

% In recent years, significant amount of progress has been made on Byzantine faulty tolerant distributed \emph{statistical parameter learning}~\cite{bernstein2018signsgd, damaskinos2018asynchronous, blanchard2017machine, cao2018distributed, chen2017distributed, alistarh2018byzantine, data2018data, xie2018generalized}. In~\cite{blanchard2017machine, xie2018generalized, damaskinos2018asynchronous, cao2018distributed, data2018data, bernstein2018signsgd} the agents assume the role of workers in the parallelization of the (stochastic) gradient descent method and therefore, agents have access to all the data points. In~\cite{data2018data}, the authors propose a data encoding scheme for tolerating Byzantine faulty workers. Whereas,~\cite{blanchard2017machine, xie2018generalized, damaskinos2018asynchronous, cao2018distributed, bernstein2018signsgd} rely on filters to ``robustify" the original distributed stochastic gradient descent method. In~\cite{chen2017distributed, yin2018byzantine,alistarh2018byzantine}, the agents have distributed data points and responses, however it is assumed that all the agents choose their data points and responses following a common probability distribution. Thus, the filtering (or encoding) techniques proposed in these papers are not guaranteed to be effective for the considered problem setting where no assumptions are made on the probability distribution of agents' data points. Moreover, we are interested in deterministic regression algorithms that compute $w^*$ in a deterministic manner. We also note that the computational complexity for the server in our proposed filtering techniques (both \emph{norm filtering} and \emph{norm-cap filtering}) is $O(n (d + \log n))$, which is significantly less than the filtering techniques proposed in~\cite{blanchard2017machine, chen2017distributed}. 
%Unlike the above Byzantine fault tolerant distributed learning techniques, we are interested in a deterministic solution that converges to the true parameter value $w^*$ (in absence of noise) and not an approximation, under certain conditions.


%In \cite{cao2018distributed}, the server has access to a reliable set of data points. 
%Dong et al. \cite{yin2018byzantine} evaluates two filtering algorithm; median-based gradient descent and trimmed mean base gradient descent for Byzantine fault-tolerance in distributed statistical learning where the agents draw data points from a common set. For the convergence analysis of median-based gradient descent they assume the variance of the gradients to have bounded variance (over the entire distribution), and for the case of trimmed mean gradient technique they assume the gradients to be sub-exponential.
% ~\cite{alistarh2018byzantine} assume that individual gradients are close to average of gradients of all honest agents as data points are chosen from a common set from a common distribution. Compared to these existing works in Byzantine-fault tolerant statistical learning, we do not make any stochastic assumptions on the data points of the agents nor do we require the data points to be common for all the agents.
% \subsection{Byzantine fault tolerant distributed multi-agent optimization}
% Byzantine faulty tolerant distributed multi-agent optimization has also received considerable attention in recent years~\cite{su2016fault, su2016robust, sundaram2018distributed, su2016multi, fanitabasi2018review}. The objective in that case is to compute the point of minimum of the weighted average cost of the honest agents. If the agents' costs are scalar (i.e. $\R \to \R$) then the server can achieve this objective with weights of at least $n-2f$ honest agents bounded away from zero~\cite{su2016fault, sundaram2018distributed}. This result is extended in~\cite{su2016robust} for multivariate cost functions, where the proposed technique relies on the assumption that agents' costs are weighted linear combination of finite number of convex functions. In general, this assumption does not hold for the regression problem considered in this paper. Further, it is known that the weights can not be uniform when there are non-zero number of Byzantine faulty agents in the system \emph{if} the costs are not correlated~\cite{su2016multi,sundaram2018distributed,su2016fault}. Interestingly, the necessary correlation between honest agents' costs that would admit equal (positive) weights for all the honest agents in Byzantine distributed multi-agent optimization problem remains an open problem. In this paper, we present a sufficient correlation between honest agents' costs under which the weights associated with honest agents' costs are equal and positive. Specifically, if there exists a common point of minimum for all the honest agents' costs (refer Section~\ref{sec:pf}) then the minimizer of the average cost of honest agents can be computed in presence of \emph{limited} (limits specified in Section~\ref{sec:conv_anal} and~\ref{sec:conv_algo_2}) number of Byzantine faulty agents. Moreover, the proposed algorithms solve this multi-agent optimization problem efficiently, under the aforementioned sufficient correlation. \\

% %Now, if the weights associated with the costs of honest agents are equal and positive then computing the point of minimum of the weighted average cost of honest agents solves the considered distributed regression problem.

% Authors in~\cite{yang2017byrdie} extend the results of~\cite{su2016multi} for multivariate cost functions by assuming that the original optimization problem can be split into \emph{independent} scalar sub-problems with \emph{strictly} convex objective costs. This assumption is quite strong and in general, does hold for the considered regression problem setting. Authors in \cite{xu2018robust} solve the Byzantine fault-tolerant distributed optimization problem, assuming that each and every agents' cost is \emph{strongly} convex, which implies that every honest agent can \emph{locally} compute $w^*$ in context of the considered regression problem. This assumption is quite strong (it basically trivializes the considered regression problem), and is not required for the effectiveness of our proposed algorithms. 


==> proof.tex <==
\section{Review of the Fault-Tolerance Property}
\label{sec:review}

We restate below our notation and assumptions from the main paper.

\begin{itemize}
    \item For each non-faulty agent $i$, let 
    \begin{align}
        \z^t_i = \{z^t_{i_1}, \ldots, \, z^t_{i_k}\} \label{eqn:non-f_data}
    \end{align}
    denote the collection i.i.d.~data points sampled by the agent $i$ in iteration $t$. Now, for each agent $i$ and iteration $t$ we define a random variable 
    \begin{align}
        \zeta^t_i = \left\{ \begin{array}{ccc} \z^t_i & , & \text{agent $i$ is non-faulty} \\ g^t_i & , & \text{agent $i$ is faulty}\end{array}\right. \label{eqn:def_zeta_i}
    \end{align}
    Recall that~$g^t_i$ may be an arbitrary $d$-dimensional random variable for each Byzantine faulty agent $i$. For each iteration $t$, let
    \begin{align}
        \zeta^t = \{\zeta^t_i, ~ i = 1, \ldots, \, n\}, \label{eqn:def_zeta}
    \end{align}
    and let $\E_t$ denote the expectation of a function of the collective random variables $\zeta^0, \ldots, \, \zeta^t$, given the initial estimate $w^0$. Specifically, 
    \begin{align}
        \E_t(\cdot) = \E_{\zeta^0, \ldots, \, \zeta^{t}} (\cdot), \quad \forall t \geq 0. \label{eqn:notation_exp}
    \end{align}
    \item We define a {\em fault-tolerance margin}  
    \begin{align}
        \alpha = \frac{\lambda}{2\lambda + \mu} - \frac{f}{n} \label{eqn:alpha_learn}
    \end{align}
    that determines the maximum fraction of faulty agents $f/n$ tolerable by our algorithm. Lastly, we define an upper bound for the step-size in~\eqref{eqn:algo_1},
    \begin{align}
        \overline{\eta} = \left(\frac{2(2 \lambda + \mu)n}{n^2 + (n-f)^2 \mu^2 } \right) \, \alpha. \label{eqn:step_learn}
    \end{align}
    % \item Let
    % \begin{align}
    %     \M^2 = \left(\frac{f^2 \left( 1 + \sqrt{n-f-1}\right)^2}{n^2} + \eta^2 (n-f)^2 \right) \sigma^2. \label{eqn:ss_error}
    % \end{align}
\end{itemize}
~

% Our assumptions are re-stated below.


% \[Z^t_1 ~ Z^t_2 ~ Z^t_n\]
% denote the collection of $k$ data points for iteration $t$ where each data point is chosen .  that in step S1 each iteration $t$, a non-faulty agent $i$ independently chooses a data point $z^t_i$ from probability distribution $\D$, and sends a {\em stochastic} gradient $g^t_i = \nabla \ell (w^t; z^t_i)$. As $Q(w) = \E_{z \sim \D} ~ \ell (w; z), ~ \forall w$, for every non-faulty agent $i$, 
% \[\E_{z^t_i \sim \D} ~ ( g^t_i ) = \nabla Q(w^t), \quad \forall t.\]

\begin{assumption}[Bounded variance]
\label{asp:bnd_var}
For each non-faulty agent $i$, assume that the variance of $g^t_i$ is bounded. Specifically, there exists a finite real value $\sigma$ such that for all non-faulty agent $i$,
\[\E_{\zeta^t_i} \norm{ g^t_i - \E_{\zeta^t_i} \left(g^t_i\right)}^2 \leq \sigma^2, \quad \forall t.\]
\end{assumption}

% As stated below, we also assume that the gradient of the expected loss function $\nabla Q(w)$ is Lipschitz continuous, and that the function $Q(w)$ is strongly convex~\cite{bottou2018optimization}. 

\begin{assumption}[Lipschitz continuity of gradients]
\label{asp:lip}
Assume that there exists a finite positive real value $\mu$ such that for all $w, \, w' \in \R^d$,
\begin{align*}
    \norm{\nabla Q(w) - \nabla Q(w')} \leq \mu \norm{w - w'}.
\end{align*}
\end{assumption}

\begin{assumption}[Strong convexity]
\label{asp:str_cvx}
Assume that there exists a finite positive real value $\lambda$ such that for all $w, \, w' \in \R^d$,
\begin{align*}
    \iprod{w - w'}{\nabla Q(w) - \nabla Q(w')} \geq \lambda \norm{w - w'}^2.
\end{align*}
\end{assumption}

% As noted by~\cite{bottou2018optimization}, the assumption on strong convexity of $Q(w)$ is not very restrictive in the practical scenarios of machine learning. For instance, in many situations when a convex learning model is used -- such as logistic regression or support vector machine -- it is often regularized by a strongly
% convex function. Moreover, even if the global cost $Q(w)$ is not strongly convex over the entire search space $\R^d$, it is so in the neighborhood of local minimizers. This means that our algorithm can guarantee fault-tolerance in small regions of the learning parameter search space.\\

We re-state below Theorem~\ref{thm:conv}, a key result on the fault-tolerance of our algorithm. Recall that $w^*$ denotes a minimum of the global expected loss function $Q(w)$, i.e., 
\[w^* \in \arg \min_w Q(w).\]
% The convergence of the modified algorithm presented in Section~\ref{sec:learn} is in expectation, where the notation $\E \norm{w^t - w^*}^2$ denotes the joint expectation of $\norm{w^t - w^*}^2$ over all the data points chosen by non-faulty agents up to the $t$-th iteration. That is, if $z^t$ denotes the random data points chosen by all the agents (including the faulty agents) for iteration $t$, then

% Let,
% \begin{align}
%     \eta < \overline{\eta} = \frac{2(2 \lambda + \mu)n}{n^2 + (n-f)^2 \mu^2 } \, \alpha, \label{eqn:step_learn}
% \end{align}
% then $\E \norm{w^{t} - w^*}^2$ converges linearly in the proximity of $w^*$ with rate of convergence 
% \[\rho = 1 - 2 \eta (2 \lambda + \mu) \alpha n + \eta^2 \left(n^2 + (n-f)^2 \mu^2 \right).\]
% Specifically, we obtain the following convergence result.\\

% \noindent \fbox{\begin{minipage}{0.96\textwidth}
\begin{theorem}[Restated]
\label{thm:conv}
Consider Algorithm~\ref{alg:cge}. Suppose that the Assumptions~\ref{asp:bnd_var},~\ref{asp:lip}, and~\ref{asp:str_cvx} hold true. If the fault-tolerance margin $\alpha$ is positive, and in the update law~\eqref{eqn:algo_1} the step-size $\eta_t = \eta \in \left(0, ~ \overline{\eta} \right)$ for all $t$ then 
\begin{align}
    \rho  = 1 - \left(n^2 + (n-f)^2 \mu^2 \right) \, \eta \left( \overline{\eta} - \eta \right) \in (0, ~ 1), \label{eqn:rho}
\end{align}
and, for all $t \geq 1$, 
\begin{align}
    \E_{t-1} \norm{w^{t} - w^*}^2 \leq \rho^{t} \norm{w^{0} - w^*}^2 + \left(\frac{1 - \rho^{t}}{ 1- \rho}\right) \M^2 \label{eqn:rate}
\end{align}
where
\begin{align}
    \M^2 = \left(\frac{f^2 \left( 1 + \sqrt{n-f-1}\right)^2}{n^2} + \eta^2 (n-f)^2 \right) \sigma^2. \label{eqn:ss_error}
\end{align}
% \begin{align}
%     \rho  = 1 - \left(n^2 + (n-f)^2 \mu^2 \right) \, \eta \left( \overline{\eta} - \eta \right)  \label{eqn:rho}
% \end{align}
% has a positive value less than $1$, and for all $t \geq 0$,
% \begin{align}
%     \E_{t} \norm{w^{t+1} - w^*}^2 \leq \rho^{t+1} \norm{w^{0} - w^*}^2 + \left(\frac{1 - \rho^{t+1}}{ 1- \rho}\right) \M^2.\label{eqn:rate}
% \end{align}
% where $w^*$ is as defined in~\eqref{eqn:obj}.
% $$ \rho_f(\eta) = 1 - \eta n \, \left(2 (\lambda + 2\mu) \alpha - \eta n \mu^2 \right) \in [0, 1), \text{ and } $$
\end{theorem}

Before we proceed to our proof of Theorem~\ref{thm:conv}, we restate below Corollary~\ref{cor:learn} along with its proof. Recall that notation $Pr(\cdot)$ denotes the probability of an event. 

% \noindent \fbox{\begin{minipage}{0.96\textwidth}
\begin{corollary}[Restated]
\label{cor:learn}
Consider our iterative algorithm. If the conditions stated in Theorem~\ref{thm:conv} hold true then
% tu Assumptions~\ref{asp:bnd_var}-\ref{asp:str_cvx} hold true, the fault-tolerance margin $\alpha$ is positive, and the step-size $\eta_t$ in~\eqref{eqn:algo_1} has a constant positive real value $\eta$ for all $t$. If $\eta < \overline{\eta}$ then 
for every positive real value $\epsilon$,
\[\lim_{t \to \infty} Pr \left( \norm{w^t - w^*}^2 \leq \epsilon \right) \geq 1 - \frac{1}{\epsilon} ~ \left( \frac{\M^2}{1 - \rho}\right). \]
\end{corollary}
\begin{proof}
Note, from Markov's inequality~\cite{mohri2018foundations}, that for an arbitrary positive real value $\epsilon$,
\begin{align}
    Pr \left( \norm{w^{t+1} - w^*}^2 \geq \epsilon \right) \leq \frac{\E_{t} \norm{w^{t+1} - w^*}^2 }{\epsilon}, \quad \forall t \geq 0. \label{eqn:markov}
\end{align}
If the conditions in Theorem~\ref{thm:conv} hold true then for all $t \geq 0$,
\begin{align*}
    \E_{t} \norm{w^{t+1} - w^*}^2 \leq \rho^{t+1} \norm{w^{0} - w^*}^2 + \left(\frac{1 - \rho^{t+1}}{ 1- \rho}\right) \M^2
\end{align*}
where $\rho \in (0, \, 1)$. Substituting from above in~\eqref{eqn:markov} we obtain, for all $t \geq 0$, that
\[ Pr \left( \norm{w^{t+1} - w^*}^2 \geq \epsilon \right) \leq \frac{1}{\epsilon} \left(\rho^{t+1} \norm{w^{0} - w^*}^2 + \left(\frac{1 - \rho^{t+1}}{ 1- \rho}\right) \M^2 \right).\]
Equivalently, 
\[Pr \left( \norm{w^{t+1} - w^*}^2 \leq \epsilon \right) \geq 1 - \frac{1}{\epsilon} \left(\rho^{t+1} \norm{w^{0} - w^*}^2 + \left(\frac{1 - \rho^{t+1}}{ 1- \rho}\right) \M^2 \right).\]
As $\rho < 1$, $\lim_{t \to \infty} \rho^t = 0$. Therefore, limiting $t$ to infinity on both sides of the above inequality proves the corollary, i.e.,
\[ \lim_{t \to \infty} Pr \left( \norm{w^{t} - w^*}^2 \leq \epsilon \right) \geq  1 -  \frac{1}{\epsilon}\left(\frac{\M^2}{ 1- \rho}\right).\]
\end{proof}

Our formal proof of Theorem~\ref{thm:conv} is presented in the subsequent section.

% \subsection{Proof of Theorem}
% Note, from~\eqref{eqn:algo_1}, that for each iteration $t$ the updated estimate $w^{t+1}$ is a function of the current estimate $w^t$, and the random variables $g^t_1, \ldots, \, g^t_n$. In case agent $i$ is non-faulty, recall from~\eqref{eqn:avg_grad} that the stochastic gradient $g^t_i$ is a function of $w^t$ and the collection of $k$ data points 
% \begin{align}
%     \z^t_i = \{z^t_{i_1}, \ldots, \, z^t_{i_k}\} \label{eqn:non-f_data}
% \end{align}
% that are independent and identically distributed (i.i.d.) by $\D$. In case agent $i$ is faulty, then $g^t_i$ is an arbitrary $d$-dimensional random variable. For each $i = 1, \ldots, \, n$, we define a random variable 
% \begin{align}
%     \zeta^t_i = \left\{ \begin{array}{ccc} \z^t_i & , & \text{$i$ is non-faulty} \\ ~\\ g^t_i & , & \text{$i$ is faulty}\end{array}\right. \label{eqn:def_zeta_i}
% \end{align}
% Let, 
% \begin{align}
%     \zeta^t = \left\{\zeta^t_1, \ldots, \, \zeta^t_n \right\}. \label{eqn:def_zeta}
% \end{align}
% ~


% For each agent $i$ and each iteration $t$, let $\E_{\zeta^t_i}(\cdot)$ denote the expected value of a function of the random variable $\zeta^t_i$ given the current estimate $w^t$. Similarly, for each non-faulty agent $i$, let $\E_{\z^t_i}(\cdot)$ denote the expected value of a function of the random variable $\z^t_i$ given the estimate $w^t$.\\

\input{conv_proof}



==> supplementary_experiments.tex <==
\section{Additional Experimental Results}
\label{sec:add_exp}

Other than the results we shown in the paper, experiments under various parameter settings are also conducted. Here we present the results.

% Next, we present the remaining details and outcomes of our experiments.
\subsection{Experiments with MNIST dataset}
\begin{figure}[b!]
    \centering
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{supplementary/40-agents/fault-type/fault-type-comparison-40-4.pdf}
        \caption{$f=4$}
        \label{fig:fault-40-4}
    \end{subfigure}\\
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{supplementary/40-agents/fault-type/fault-type-comparison-40-8.pdf}
        \caption{$f=8$}
        \label{fig:fault-40-8}
    \end{subfigure}\\
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{supplementary/40-agents/fault-type/fault-type-comparison-40-12.pdf}
        \caption{$f=12$}
        \label{fig:fault-40-12}
    \end{subfigure}
    \caption{\footnotesize Distributed learning of the convolutional neural network $\mathsf{LeNet}$ for the MNIST dataset using the D-SGD method with different gradient-filters (represented by different colors) to tolerate different numbers of faulty agents in the system. The training losses and the testing precisions evaluated by the server after $0$ to $500$ iterations (or steps) of the different learning algorithms are plotted in the first and the second rows, respectively. Different columns contain the results for different types of faults simulated by the faulty agents. Here, the data batch size $k=64$.}
    \label{fig:mnist-fault-comparison-01}
\end{figure}

We conducted series of experiments with MNIST dataset and 40 agents in the system while changing the number of faulty agents in the system from 1 to 12. Here we selectively present results with $f=4,\,8$, and $12$, or $10\%,\,20\%$, and $30\%$ of faulty agents in the system respectively, shown in Figure~\ref{fig:mnist-fault-comparison-01}. Note that theoretically, MoM with $b=2$ can only tolerate less than 8 fault agents in a 40-agent system, which is also supported by some experimental results.\\ 

We also observe that \textit{norm-confusing} is a difficult fault type for CGE, as its performance deteriorates fast when number of faulty agents increases, comparing to its performances when facing other fault types, which are comparable to other state-of-the-art gradient filters no matter how many faulty agents. Need to note that when facing \textit{norm-confusing}, instead of being unable to converge, CGE only converges slower.

\subsection{Experiments with CIFAR-10 dataset}

\begin{figure}[tb!]
    \centering
    \includegraphics[width=\linewidth]{supplementary/40-agents/cifar/cifar-comparison-2.pdf}
    \caption{Distributed learning of $\mathsf{LeNet}$ for CIFAR-10 dataset using the D-SGD method with batch size $k=64$ and the different gradient-filters (represented using different colors) in the presence of $f = 4$ faulty agents exhibiting different Byzantine faults.}
    \label{fig:cifar-fault-comparison-01}
\end{figure}

\begin{figure}[tb!]
    \centering
    \includegraphics[width=0.6\linewidth]{supplementary/40-agents/cifar/averaging-cifar-comparison-3.pdf}
    \caption{Average training losses and testing precisions evaluated between $1175$ to $1200$ steps of the D-SGD method with CGE gradient-filter for distributed learning of the neural network $\mathsf{LeNet}$ (for the CIFAR-10 dataset) in the presence of different number of faulty agents $f$ (represented by different colors) when applying temporal averaging of stochastic for different values of $\alpha$. \emph{no ave.} indicates the case when no averaging is not used. Here, the data batch-size $k = 64$.}
    \label{fig:cifar-averaging-01}
\end{figure}

We further conducted our experiments with CIFAR-10 dataset and 40 agents in the system. We trained an extra 700 steps with batch size $k=64$ and $f=4$ faulty agents in the system, with results shown in Figure~\ref{fig:cifar-fault-comparison-01}. We also applied our proposed temporal averaging scheme. As is shown in Figure~\ref{fig:cifar-averaging-01}, with temporal averaging scheme, for classification task on CIFAR-10 dataset, better performance can be achieved as well, if trained with same number of steps.\\

